Peptide Sequencing Via Protein Language Models

We introduce a protein language model for determining the complete sequence of a peptide based on measurement of a limited set of amino acids. To date, protein sequencing relies on mass spectrometry, with some novel edman degregation based platforms able to sequence non-native peptides. Current protein sequencing techniques face limitations in accurately identifying all amino acids, hindering comprehensive proteome analysis. Our method simulates partial sequencing data by selectively masking amino acids that are experimentally difficult to identify in protein sequences from the UniRef database. This targeted masking mimics real-world sequencing limitations. We then modify and finetune a ProtBert derived transformer-based model, for a new downstream task predicting these masked residues, providing an approximation of the complete sequence. Evaluating on three bacterial Escherichia species, we achieve per-amino-acid accuracy up to 90.5% when only four amino acids ([KCYM]) are known. Structural assessment using AlphaFold and TM-score validates the biological relevance of our predictions. The model also demonstrates potential for evolutionary analysis through cross-species performance. This integration of simulated experimental constraints with computational predictions offers a promising avenue for enhancing protein sequence analysis, potentially accelerating advancements in proteomics and structural biology by providing a probabilistic reconstruction of the complete protein sequence from limited experimental data.

==> Alphafold/A0A066T1W5.tex <==


ID = A0A066T1W5



Description = Cystathionine beta-lyase n=31 Tax=Bacteria TaxID=2 RepID=A0A066T1W5\_ECOLX

Length = 395 (aa)

Predicted matches = 309 / 352 (87.78\%)

TM-score = 0.8978

Superposition in the TM-score: Length(d<5.0)= 352

\includegraphics[width=\textwidth]{Alphafold/A0A066T1W5.png}
\textbf{Left:} AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). \textbf{Center:} AlphaFold structure of predicted sequence. \textbf{Right:} AlphaFold structure of UniProtKB sequence.\\ \\

Alignment between predicted sequence and UniProtKB sequence:\\

{
\begin{spacing}{0.5}
\ttfamily
\fontsize{6.5}{11}\selectfont
\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{S}\textcolor{black}{K}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{E\ }\textcolor{green}{A}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{C\ }\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{S}\textcolor{black}{K}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{E\ }\textcolor{green}{A}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{C\ }\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A\ }\\
\\
\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{F}\textcolor{black}{C}\textcolor{green}{S}\textcolor{black}{K\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{green}{W}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{T\ }\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{G\ }\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{K\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{I\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{F}\textcolor{black}{C}\textcolor{green}{S}\textcolor{black}{K\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{green}{W}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{T\ }\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{G\ }\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{K\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{I\ }\\
\\
\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{W\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{Y\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{S\ }\textcolor{red}{I}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{H\ }\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{W\ }\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{red}{S\ }\textcolor{red}{N}\textcolor{green}{E}\textcolor{green}{E}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{N\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{W\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{Y\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{S\ }\textcolor{red}{L}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{H\ }\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{W\ }\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{red}{N\ }\textcolor{red}{D}\textcolor{green}{E}\textcolor{green}{E}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{N\ }\\
\\
\textcolor{green}{F}\textcolor{green}{S}\textcolor{red}{R}\textcolor{green}{F}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{red}{D}\textcolor{green}{W\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{red}{V}\textcolor{green}{S}\textcolor{red}{T}\textcolor{red}{D}\textcolor{green}{L}\textcolor{red}{E}\textcolor{red}{T\ }\textcolor{red}{S}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{H}\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{E}\textcolor{red}{L}\textcolor{red}{I\ }\textcolor{red}{A}\textcolor{red}{W}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{V}\textcolor{green}{S}\textcolor{red}{N}\textcolor{red}{E}\textcolor{red}{E\ }\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{R}\textcolor{green}{H}\textcolor{green}{I}\textcolor{red}{N}\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{E\ }\textcolor{red}{G}\textcolor{green}{D}\textcolor{red}{G}\textcolor{red}{D}\textcolor{green}{A}\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{V}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{green}{F}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{red}{S}\textcolor{green}{W\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{red}{E}\textcolor{green}{S}\textcolor{red}{L}\textcolor{red}{I}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{N\ }\textcolor{red}{Q}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{H}\textcolor{red}{I}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{R}\textcolor{red}{P\ }\textcolor{red}{Q}\textcolor{red}{G}\textcolor{black}{K}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{F}\textcolor{green}{S}\textcolor{red}{G}\textcolor{red}{T}\textcolor{red}{L\ }\textcolor{red}{I}\textcolor{red}{R}\textcolor{red}{L}\textcolor{green}{H}\textcolor{green}{I}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{E}\textcolor{red}{D}\textcolor{red}{V\ }\textcolor{red}{D}\textcolor{green}{D}\textcolor{red}{L}\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{D}\textcolor{red}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{red}{F}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{V} \\
\end{spacing}
}
\vspace{5pt}
\hrule


==> Alphafold/A0A0D6GPE6.tex <==


ID = A0A0D6GPE6



Description = Tail fiber assembly protein n=16 Tax=Escherichia coli TaxID=562 RepID=A0A0D6GPE6\_ECOLX

Length = 200 (aa)

Predicted matches = 155 / 176 (88.07\%)

TM-score = 0.9868

Superposition in the TM-score: Length(d<5.0)= 200

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A0D6GPE6.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{N}\textcolor{black}{K}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{S}\textcolor{red}{E}\textcolor{green}{L\ }\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{E}\textcolor{black}{Y\ }\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{S}\textcolor{red}{N}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{I\ }\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{L\ }\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{S}\textcolor{red}{A}\textcolor{red}{D}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{S\ }\textcolor{green}{W}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{G}\textcolor{red}{D}\textcolor{red}{T\ }\textcolor{black}{K}\textcolor{red}{E}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{P\ }\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{D}\textcolor{black}{K}\textcolor{green}{A}\textcolor{red}{I}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{S}\textcolor{red}{G}\textcolor{green}{L\ }\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{E}\textcolor{black}{Y\ }\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{S}\textcolor{red}{S}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{V\ }\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{L\ }\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{S}\textcolor{red}{V}\textcolor{red}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{S\ }\textcolor{green}{W}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{G}\textcolor{red}{E}\textcolor{red}{S\ }\textcolor{black}{K}\textcolor{red}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{P\ }\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T\ }\\
\\
\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{W}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{W\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{Q\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I\ }\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{red}{T}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{E}\textcolor{red}{L}\textcolor{red}{N}\textcolor{green}{T}\textcolor{red}{S}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{D}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{P\ }\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{P}\textcolor{red}{S}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{W}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{W\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{Q\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I\ }\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{red}{A}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{Q}\textcolor{red}{A}\textcolor{red}{E}\textcolor{green}{T}\textcolor{red}{T}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{N}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{P\ }\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{P}\textcolor{red}{E}\textcolor{green}{A\ }\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A0H2V6J2.tex <==


ID = A0A0H2V6J2



Description = Putative tail fiber component K of prophage n=1 Tax=Escherichia coli O6:H1 TaxID=199310 RepID=A0A0H2V6J2\_ECOL6

Length = 232 (aa)

Predicted matches = 181 / 206 (87.86\%)

TM-score = 0.9794

Superposition in the TM-score: Length(d<5.0)= 229

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A0H2V6J2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{R}\textcolor{red}{S}\textcolor{red}{R}\textcolor{red}{N}\textcolor{black}{C}\textcolor{red}{F}\textcolor{red}{A}\textcolor{green}{V}\textcolor{red}{L\ }\textcolor{red}{V}\textcolor{green}{T}\textcolor{red}{S}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{red}{D}\textcolor{red}{D\ }\textcolor{black}{C}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{A\ }\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{W}\textcolor{red}{F}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{Q\ }\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{G}\textcolor{red}{E}\textcolor{green}{I}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{R}\textcolor{black}{C\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{E\ }\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{F\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{P}\textcolor{red}{A}\textcolor{red}{E}\textcolor{red}{S}\textcolor{black}{C}\textcolor{red}{G}\textcolor{red}{L}\textcolor{green}{V}\textcolor{red}{V\ }\textcolor{red}{R}\textcolor{green}{T}\textcolor{red}{P}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{red}{I}\textcolor{red}{P\ }\textcolor{black}{C}\textcolor{green}{V}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{A\ }\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{A}\textcolor{red}{P}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{W}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{Q\ }\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{I}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{R}\textcolor{black}{C\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{E\ }\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{F\ }\\
\\
\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{E\ }\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{W\ }\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{red}{I\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{G}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{A\ }\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{G\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{H}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{W\ }\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{H\ }\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{G\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{E\ }\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{W\ }\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{red}{V\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{G}\textcolor{red}{S}\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{P\ }\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{G\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{H}\textcolor{red}{I}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{W\ }\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{H\ }\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{G\ }\\
\\
\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{black}{C}\textcolor{black}{M}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{black}{C}\textcolor{black}{M}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A0L7AAG3.tex <==


ID = A0A0L7AAG3



Description = 4-diphosphocytidyl-2-C-methyl-D-erythritol kinase n=1 Tax=Escherichia coli TaxID=562 RepID=A0A0L7AAG3\_ECOLX

Length = 283 (aa)

Predicted matches = 206 / 260 (79.23\%)

TM-score = 0.9326

Superposition in the TM-score: Length(d<5.0)= 273

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A0L7AAG3.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{A}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{Q\ }\textcolor{green}{R}\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{red}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{E}\textcolor{red}{P}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{D\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{P}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{G}\textcolor{red}{H}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{red}{N}\textcolor{red}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{P}\textcolor{black}{M\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{P}\textcolor{green}{L}\textcolor{red}{R}\textcolor{red}{P}\textcolor{green}{G}\textcolor{red}{R}\textcolor{red}{D}\textcolor{green}{N\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{S}\textcolor{red}{P}\textcolor{green}{A}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{Q\ }\textcolor{green}{R}\textcolor{red}{S}\textcolor{green}{D}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{red}{I}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{E}\textcolor{red}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{red}{A}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{A\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{red}{E}\textcolor{red}{I}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{P}\textcolor{black}{M\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{G}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{G}\textcolor{green}{G}\textcolor{red}{S}\textcolor{red}{S}\textcolor{green}{N\ }\\
\\
\textcolor{red}{P}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{A\ }\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{E}\textcolor{black}{C}\textcolor{red}{S}\textcolor{red}{H}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{E}\textcolor{red}{Q\ }\textcolor{red}{V}\textcolor{green}{A}\textcolor{red}{R}\textcolor{black}{M}\textcolor{red}{S}\textcolor{red}{G}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{R}\textcolor{red}{S\ }\textcolor{red}{V}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{G}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{R}\textcolor{red}{R}\textcolor{green}{H}\textcolor{red}{G\ }\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{red}{E}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{D}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{red}{I}\textcolor{red}{P}\textcolor{green}{H}\textcolor{red}{N}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{I}\textcolor{red}{H}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{R\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{N}\textcolor{red}{H\ }\textcolor{red}{L}\textcolor{red}{W}\textcolor{red}{Q}\textcolor{black}{C}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{E\ }\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{E}\textcolor{black}{M}\textcolor{red}{G}\textcolor{red}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{A\ }\textcolor{red}{D}\textcolor{red}{V}\textcolor{red}{P}\textcolor{red}{V}\textcolor{red}{F}\textcolor{green}{V}\textcolor{green}{R}\textcolor{red}{G}\textcolor{green}{H}\textcolor{red}{A\ }\textcolor{green}{A}\textcolor{red}{F}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V}\textcolor{red}{G}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{red}{V}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{W}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{red}{V}\textcolor{red}{A}\textcolor{green}{H}\textcolor{red}{P}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{I}\textcolor{red}{F}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{R\ }\\
\\
\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{red}{P}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{L}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{red}{E}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{L}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A152XFT4.tex <==


ID = A0A152XFT4



Description = DUF3251 domain-containing protein n=4 Tax=Escherichia coli TaxID=562 RepID=A0A152XFT4\_ECOLX

Length = 179 (aa)

Predicted matches = 129 / 164 (78.66\%)

TM-score = 0.6095

Superposition in the TM-score: Length(d<5.0)= 107

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A152XFT4.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{Q\ }\textcolor{red}{Q}\textcolor{green}{G}\textcolor{green}{S}\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{A}\textcolor{black}{C\ }\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{black}{K\ }\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{red}{N\ }\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{D}\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{I}\textcolor{red}{Q}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{P\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{L\ }\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{A}\textcolor{black}{C\ }\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{black}{K\ }\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{red}{I\ }\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{D}\textcolor{red}{I}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{I}\textcolor{red}{E}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{P\ }\\
\\
\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{E}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{F\ }\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{red}{L\ }\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{T}\textcolor{green}{S}\textcolor{red}{D}\textcolor{red}{P}\textcolor{green}{A}\textcolor{red}{T}\textcolor{red}{L\ }\textcolor{green}{D}\textcolor{red}{P}\textcolor{green}{D}\textcolor{red}{F}\textcolor{green}{P}\textcolor{red}{T}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{black}{K}\textcolor{red}{R\ }\textcolor{red}{S}\textcolor{green}{S}\textcolor{black}{M}\textcolor{red}{A}\textcolor{red}{D}\textcolor{red}{R}\textcolor{red}{F}\textcolor{red}{Q}\textcolor{red}{A}\textcolor{red}{E\ }\textcolor{red}{V}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{F}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{red}{T}\textcolor{black}{M}\textcolor{red}{H}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{E}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{red}{Q}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{F\ }\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{I}\textcolor{red}{N}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{red}{I\ }\textcolor{red}{N}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{A}\textcolor{green}{S}\textcolor{red}{V}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{S\ }\textcolor{green}{D}\textcolor{red}{V}\textcolor{green}{D}\textcolor{red}{I}\textcolor{green}{P}\textcolor{red}{L}\textcolor{green}{Q}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{G\ }\textcolor{red}{I}\textcolor{green}{S}\textcolor{black}{M}\textcolor{red}{D}\textcolor{red}{Q}\textcolor{red}{L}\textcolor{red}{G}\textcolor{red}{F}\textcolor{red}{L}\textcolor{red}{R\ }\textcolor{red}{I}\textcolor{red}{H}\textcolor{red}{D}\textcolor{red}{I}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{red}{V}\textcolor{black}{M}\textcolor{red}{Q}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A152XIX0.tex <==


ID = A0A152XIX0



Description = Aldose epimerase n=5 Tax=Escherichia coli TaxID=562 RepID=A0A152XIX0\_ECOLX

Length = 300 (aa)

Predicted matches = 221 / 265 (83.40\%)

TM-score = 0.9667

Superposition in the TM-score: Length(d<5.0)= 296

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A152XIX0.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{N}\textcolor{black}{M}\textcolor{green}{H}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{C\ }\textcolor{black}{Y}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{red}{E}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{W\ }\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{V\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{N}\textcolor{black}{M}\textcolor{green}{H}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{C\ }\textcolor{black}{Y}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{red}{D}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{W\ }\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{V\ }\\
\\
\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{F}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{red}{H}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{H}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{green}{V}\textcolor{green}{D}\textcolor{red}{E}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{red}{N}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{E}\textcolor{red}{N}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{T}\textcolor{red}{F}\textcolor{red}{L}\textcolor{green}{H}\textcolor{red}{H}\textcolor{red}{I}\textcolor{red}{D\ }\textcolor{red}{E}\textcolor{red}{R}\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{N}\textcolor{red}{W}\textcolor{red}{T}\textcolor{red}{E}\textcolor{red}{G}\textcolor{black}{K\ }\textcolor{red}{T}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{R}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{F\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{F}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{H}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{green}{V}\textcolor{green}{D}\textcolor{red}{D}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{red}{E}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{E}\textcolor{red}{H}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{T}\textcolor{red}{L}\textcolor{red}{H}\textcolor{green}{H}\textcolor{red}{V}\textcolor{red}{D}\textcolor{red}{E\ }\textcolor{red}{L}\textcolor{red}{N}\textcolor{red}{L}\textcolor{red}{N}\textcolor{red}{F}\textcolor{red}{T}\textcolor{red}{R}\textcolor{red}{A}\textcolor{red}{T}\textcolor{black}{K\ }\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{T}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{F\ }\\
\\
\textcolor{black}{K}\textcolor{red}{E}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{R}\textcolor{green}{W}\textcolor{green}{E}\textcolor{black}{M}\textcolor{red}{D\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{red}{R}\textcolor{red}{H}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{E}\textcolor{red}{D\ }\textcolor{red}{E}\textcolor{green}{L}\textcolor{black}{C}\textcolor{black}{C}\textcolor{red}{F}\textcolor{red}{R}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{red}{I}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{Q\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{P\ }\textcolor{green}{P}\textcolor{red}{N}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{E}\textcolor{red}{S}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{P}\textcolor{green}{H}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{L}\textcolor{green}{W}\textcolor{green}{E}\textcolor{black}{M}\textcolor{red}{T\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{red}{H}\textcolor{red}{P}\textcolor{red}{Q}\textcolor{red}{H}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{V\ }\textcolor{red}{S}\textcolor{green}{L}\textcolor{black}{C}\textcolor{black}{C}\textcolor{red}{D}\textcolor{red}{Q}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{red}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{Q\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{P\ }\textcolor{green}{P}\textcolor{red}{D}\textcolor{green}{A}\textcolor{red}{F}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{red}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{red}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{H}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{black}{K\ }\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A1M2R6U0.tex <==


ID = A0A1M2R6U0



Description = YdeA protein n=20 Tax=Enterobacteriaceae TaxID=543 RepID=A0A1M2R6U0\_ECOLX

Length = 196 (aa)

Predicted matches = 154 / 187 (82.35\%)

TM-score = 0.7225

Superposition in the TM-score: Length(d<5.0)= 171

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A1M2R6U0.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{Q\ }\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{R\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{N\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{red}{T}\textcolor{green}{G}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{P\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{red}{G}\textcolor{red}{R}\textcolor{red}{R}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{red}{R}\textcolor{red}{R\ }\textcolor{green}{Q}\textcolor{red}{Q}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{E}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{P\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{A\ }\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{R\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{N\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{red}{A}\textcolor{green}{G}\textcolor{red}{W}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{P\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{red}{E}\textcolor{red}{L}\textcolor{red}{T}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{red}{P}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{R}\textcolor{red}{A}\textcolor{red}{E\ }\textcolor{green}{Q}\textcolor{red}{R}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{P\ }\\
\\
\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{E\ }\textcolor{red}{R}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{R\ }\textcolor{green}{G}\textcolor{red}{G}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{R\ }\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{L\ }\textcolor{green}{R}\textcolor{red}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{red}{H}\textcolor{green}{L\ }\textcolor{red}{V}\textcolor{green}{V}\textcolor{red}{L}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{H\ }\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{I\ }\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{S}\textcolor{red}{S}\textcolor{red}{V}\textcolor{green}{P}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{V}\textcolor{green}{E\ }\textcolor{red}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{R\ }\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{S\ }\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{G\ }\textcolor{green}{R}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{R}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{red}{P}\textcolor{green}{L\ }\textcolor{red}{E}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{H\ }\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{V\ }\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{S}\textcolor{red}{V}\textcolor{red}{T}\textcolor{green}{P}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A1X3J5V0.tex <==


ID = A0A1X3J5V0



Description = Flagellar protein export ATPase FliI n=1 Tax=Escherichia coli TA447 TaxID=656447 RepID=A0A1X3J5V0\_ECOLX

Length = 445 (aa)

Predicted matches = 327 / 397 (82.37\%)

TM-score = 0.9334

Superposition in the TM-score: Length(d<5.0)= 407

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A1X3J5V0.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{N}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{E\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{E}\textcolor{red}{V\ }\textcolor{red}{S}\textcolor{red}{D}\textcolor{red}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{red}{D}\textcolor{red}{A}\textcolor{red}{G}\textcolor{red}{V\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\\
\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{E\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{E}\textcolor{red}{S\ }\textcolor{red}{W}\textcolor{red}{L}\textcolor{red}{G}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{red}{N}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{G\ }\\
\\
\textcolor{green}{E}\textcolor{red}{V}\textcolor{red}{N}\textcolor{red}{I}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{D}\textcolor{red}{E}\textcolor{black}{K\ }\textcolor{red}{S}\textcolor{red}{R}\textcolor{red}{G}\textcolor{red}{V}\textcolor{red}{S}\textcolor{red}{G}\textcolor{red}{Q}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{T\ }\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{A}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{R}\textcolor{red}{I}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{red}{G}\textcolor{green}{P}\textcolor{red}{A}\textcolor{green}{D}\textcolor{red}{G}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{G\ }\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{E\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{H}\textcolor{red}{I}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{red}{E}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{V\ }\\
\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{E}\textcolor{red}{P}\textcolor{red}{L}\textcolor{red}{D}\textcolor{red}{S}\textcolor{black}{K}\textcolor{red}{G}\textcolor{red}{R}\textcolor{red}{L}\textcolor{black}{K\ }\textcolor{red}{G}\textcolor{red}{N}\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{P}\textcolor{red}{P}\textcolor{green}{L}\textcolor{red}{P}\textcolor{red}{P\ }\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{N}\textcolor{red}{P}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{R}\textcolor{red}{S}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{red}{E}\textcolor{green}{P}\textcolor{red}{L}\textcolor{green}{D}\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{G\ }\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{E\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{H}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{L}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{V\ }\\
\\
\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{red}{Q}\textcolor{red}{T}\textcolor{black}{K}\textcolor{red}{I}\textcolor{red}{A}\textcolor{green}{E}\textcolor{red}{A}\textcolor{black}{C}\textcolor{green}{H}\textcolor{red}{A\ }\textcolor{red}{A}\textcolor{red}{G}\textcolor{red}{T}\textcolor{red}{D}\textcolor{red}{D}\textcolor{red}{E}\textcolor{red}{R}\textcolor{black}{C}\textcolor{red}{S}\textcolor{red}{A\ }\textcolor{red}{S}\textcolor{green}{V}\textcolor{red}{G}\textcolor{red}{V}\textcolor{red}{D}\textcolor{red}{L}\textcolor{green}{D}\textcolor{red}{I}\textcolor{red}{V}\textcolor{red}{L\ }\textcolor{green}{R}\textcolor{black}{Y}\textcolor{red}{W}\textcolor{black}{M}\textcolor{red}{R}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A\ }\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{G}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{K\ }\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{E}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{red}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{Y\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{red}{R}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{T}\textcolor{green}{E}\textcolor{red}{L}\textcolor{black}{C}\textcolor{green}{H}\textcolor{red}{S\ }\textcolor{red}{I}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{W}\textcolor{red}{F}\textcolor{red}{R}\textcolor{red}{D}\textcolor{black}{C}\textcolor{red}{G}\textcolor{red}{H\ }\textcolor{red}{H}\textcolor{green}{V}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{V}\textcolor{green}{D}\textcolor{red}{S}\textcolor{red}{L}\textcolor{red}{T\ }\textcolor{green}{R}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{black}{M}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{L}\textcolor{green}{G}\textcolor{red}{E}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{K\ }\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{Y\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V\ }\\
\\
\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{R}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I\ }\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{R}\textcolor{black}{C}\textcolor{black}{M\ }\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{green}{S}\textcolor{green}{R}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{P}\textcolor{red}{E}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{R}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I\ }\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{R}\textcolor{black}{C}\textcolor{black}{M\ }\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{green}{S}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{P}\textcolor{red}{T}\textcolor{green}{A\ }\\
\\
\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{Q}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{Q}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A271R208.tex <==


ID = A0A271R208



Description = DUF1198 domain-containing protein n=3 Tax=Enterobacteriaceae TaxID=543 RepID=A0A271R208\_ECOLX

Length = 150 (aa)

Predicted matches = 108 / 137 (78.83\%)

TM-score = 0.7901

Superposition in the TM-score: Length(d<5.0)= 129

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A271R208.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{W}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{D}\textcolor{green}{V\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{Q\ }\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{V}\textcolor{red}{R}\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{W}\textcolor{red}{G\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{D}\textcolor{red}{L}\textcolor{green}{S}\textcolor{red}{D}\textcolor{green}{Q}\textcolor{red}{Q\ }\textcolor{green}{L}\textcolor{red}{I}\textcolor{red}{Q}\textcolor{red}{V}\textcolor{green}{H}\textcolor{green}{R}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{A}\textcolor{black}{K\ }\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{R}\textcolor{red}{A}\textcolor{red}{E}\textcolor{red}{S}\textcolor{red}{A}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{W}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{V\ }\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{Q\ }\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{green}{V}\textcolor{red}{L}\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{W}\textcolor{red}{Q\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{red}{V}\textcolor{green}{D}\textcolor{red}{G}\textcolor{green}{S}\textcolor{red}{E}\textcolor{green}{Q}\textcolor{red}{N\ }\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{R}\textcolor{red}{W}\textcolor{green}{H}\textcolor{green}{R}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{Q}\textcolor{black}{K\ }\textcolor{red}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{I}\textcolor{red}{T}\textcolor{red}{D}\textcolor{green}{A\ }\\
\\
\textcolor{red}{L}\textcolor{green}{V}\textcolor{red}{L}\textcolor{red}{D}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{G}\textcolor{red}{F}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{red}{N}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{H\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\\
\textcolor{red}{Q}\textcolor{green}{V}\textcolor{red}{R}\textcolor{red}{Q}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{G}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{red}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{H\ }\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A2A7M6X5.tex <==


ID = A0A2A7M6X5



Description = Helix-turn-helix-type transcriptional regulator n=1 Tax=Escherichia coli TaxID=562 RepID=A0A2A7M6X5\_ECOLX

Length = 243 (aa)

Predicted matches = 176 / 219 (80.37\%)

TM-score = 0.6734

Superposition in the TM-score: Length(d<5.0)= 159

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A2A7M6X5.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{K}\textcolor{red}{Q}\textcolor{green}{W}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{red}{G}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{red}{D}\textcolor{green}{T}\textcolor{red}{E}\textcolor{green}{D}\textcolor{green}{D\ }\textcolor{green}{W}\textcolor{red}{I}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{E}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{S\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{E\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{K}\textcolor{red}{R}\textcolor{green}{W}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{red}{E}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{red}{N}\textcolor{green}{T}\textcolor{red}{Q}\textcolor{green}{D}\textcolor{green}{D\ }\textcolor{green}{W}\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{E}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{S\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{E\ }\\
\\
\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{S\ }\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{red}{T\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{K\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{W\ }\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{red}{T}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{W}\textcolor{red}{G\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{G}\textcolor{green}{W\ }\textcolor{green}{H}\textcolor{green}{I}\textcolor{red}{V}\textcolor{green}{V}\textcolor{red}{S}\textcolor{red}{H}\textcolor{green}{D}\textcolor{green}{P}\textcolor{red}{A}\textcolor{red}{S\ }\textcolor{red}{T}\textcolor{green}{P}\textcolor{red}{S}\textcolor{red}{S}\textcolor{red}{R}\textcolor{red}{R}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{R}\textcolor{red}{A\ }\textcolor{red}{P}\textcolor{red}{P}\textcolor{red}{S}\textcolor{red}{P}\textcolor{red}{D}\textcolor{red}{I}\textcolor{red}{S}\textcolor{red}{A}\textcolor{red}{D}\textcolor{red}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\\
\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{S\ }\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{red}{A\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{K\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{W\ }\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{red}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{W}\textcolor{red}{L\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{red}{W}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{W\ }\textcolor{green}{H}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{V}\textcolor{red}{L}\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{P}\textcolor{red}{I}\textcolor{red}{E\ }\textcolor{red}{S}\textcolor{green}{P}\textcolor{red}{R}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{L}\textcolor{red}{F}\textcolor{red}{P}\textcolor{red}{T}\textcolor{red}{Q\ }\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{I}\textcolor{red}{V}\textcolor{red}{W}\textcolor{red}{T}\textcolor{red}{G}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{P\ }\\
\\
\textcolor{red}{I}\textcolor{red}{G}\textcolor{red}{A}\textcolor{red}{P}\textcolor{green}{N}\textcolor{red}{S}\textcolor{red}{T}\textcolor{green}{L}\textcolor{red}{H}\textcolor{red}{T\ }\textcolor{green}{W}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{F\ }\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{P}\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{red}{T}\textcolor{red}{R}\textcolor{red}{R}\textcolor{red}{Q}\textcolor{green}{N}\textcolor{red}{E}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{red}{H\ }\textcolor{green}{W}\textcolor{red}{G}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{F\ }\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{P}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A2P9E0I9.tex <==


ID = A0A2P9E0I9



Description = Sensor protein n=22 Tax=Bacteria TaxID=2 RepID=A0A2P9E0I9\_ECOLX

Length = 491 (aa)

Predicted matches = 377 / 447 (84.34\%)

TM-score = 0.8565

Superposition in the TM-score: Length(d<5.0)= 447

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A2P9E0I9.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{H}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{P}\textcolor{red}{F}\textcolor{red}{V}\textcolor{green}{R}\textcolor{red}{D}\textcolor{red}{L\ }\textcolor{green}{S}\textcolor{red}{P}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{F}\textcolor{red}{R\ }\textcolor{red}{F}\textcolor{red}{F}\textcolor{red}{A}\textcolor{green}{T}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{R}\textcolor{red}{S\ }\textcolor{red}{S}\textcolor{red}{A}\textcolor{green}{W}\textcolor{red}{Q}\textcolor{black}{M}\textcolor{red}{A}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{V\ }\textcolor{black}{K}\textcolor{green}{H}\textcolor{red}{D}\textcolor{red}{I}\textcolor{green}{E}\textcolor{red}{H}\textcolor{red}{R}\textcolor{green}{V}\textcolor{red}{Q}\textcolor{red}{E\ }\textcolor{red}{H}\textcolor{red}{I}\textcolor{red}{N}\textcolor{red}{T}\textcolor{red}{I}\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{P}\textcolor{red}{Q}\textcolor{red}{L\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{V}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{D}\textcolor{red}{D\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{I}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{P}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{N\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{red}{T}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{A\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{H}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{P}\textcolor{red}{S}\textcolor{red}{R}\textcolor{green}{R}\textcolor{red}{P}\textcolor{red}{F\ }\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{F}\textcolor{red}{I\ }\textcolor{red}{S}\textcolor{red}{L}\textcolor{red}{S}\textcolor{green}{T}\textcolor{red}{I}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{F}\textcolor{red}{I}\textcolor{red}{A\ }\textcolor{red}{F}\textcolor{red}{T}\textcolor{green}{W}\textcolor{red}{F}\textcolor{black}{M}\textcolor{red}{L}\textcolor{red}{H}\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{E\ }\textcolor{black}{K}\textcolor{green}{H}\textcolor{red}{F}\textcolor{red}{A}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{red}{D}\textcolor{green}{V}\textcolor{red}{S}\textcolor{red}{D\ }\textcolor{red}{L}\textcolor{red}{Q}\textcolor{red}{Q}\textcolor{red}{I}\textcolor{red}{S}\textcolor{red}{T}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{R\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{A}\textcolor{green}{D}\textcolor{red}{P}\textcolor{green}{D}\textcolor{red}{E\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{V}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{L\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{G}\textcolor{red}{E}\textcolor{green}{V}\textcolor{red}{L}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{red}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{A\ }\\
\\
\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{S\ }\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{V}\textcolor{red}{I}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{M}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{Q\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{H}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{S\ }\textcolor{red}{R}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{M}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{Q\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{H}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{red}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{A\ }\\
\\
\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{N\ }\textcolor{green}{H}\textcolor{black}{M}\textcolor{red}{V}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{N\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{T\ }\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{N\ }\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{L\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{red}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{N\ }\textcolor{green}{H}\textcolor{black}{M}\textcolor{red}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{N\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{S\ }\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{N\ }\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{L\ }\\
\\
\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{W}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{R}\textcolor{red}{E}\textcolor{green}{F}\textcolor{red}{R\ }\textcolor{green}{R}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{Q\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{F}\textcolor{red}{D\ }\textcolor{green}{R}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{Q\ }\\
\\
\textcolor{green}{R}\textcolor{black}{K}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{G}\textcolor{red}{I\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{H\ }\textcolor{green}{H}\textcolor{red}{A}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{red}{N}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{V\ }\textcolor{red}{H}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{P}\textcolor{red}{S}\textcolor{green}{P\ }\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{black}{M}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{Q\ }\textcolor{black}{C}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\\
\textcolor{green}{R}\textcolor{black}{K}\textcolor{red}{G}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{G}\textcolor{red}{L\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{H\ }\textcolor{green}{H}\textcolor{red}{G}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{red}{E}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{V\ }\textcolor{red}{R}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{V}\textcolor{green}{P\ }\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{black}{M}\textcolor{red}{I}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{Q\ }\textcolor{black}{C}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A2T1MJ64.tex <==


ID = A0A2T1MJ64



Description = Fimbrial protein n=2 Tax=Escherichia coli TaxID=562 RepID=A0A2T1MJ64\_ECOLX

Length = 236 (aa)

Predicted matches = 183 / 212 (86.32\%)

TM-score = 0.8325

Superposition in the TM-score: Length(d<5.0)= 201

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A2T1MJ64.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{A}\textcolor{green}{V}\textcolor{black}{C}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{N\ }\textcolor{green}{N}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{black}{K\ }\textcolor{green}{F}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{R\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{V}\textcolor{black}{C}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{N\ }\textcolor{green}{N}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{black}{K\ }\textcolor{green}{F}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{R\ }\\
\\
\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{E\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{F}\textcolor{red}{R\ }\textcolor{red}{T}\textcolor{red}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{T}\textcolor{red}{G}\textcolor{red}{F}\textcolor{green}{T}\textcolor{red}{T}\textcolor{red}{F\ }\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{P}\textcolor{red}{P}\textcolor{red}{V}\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{V}\textcolor{green}{V}\textcolor{red}{R\ }\textcolor{red}{A}\textcolor{red}{N}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{red}{V}\textcolor{black}{K}\textcolor{green}{W}\textcolor{red}{V\ }\textcolor{green}{F}\textcolor{red}{G}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{N\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{P\ }\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{D}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{E\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{R}\textcolor{red}{S\ }\textcolor{red}{P}\textcolor{red}{T}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{E}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{T}\textcolor{red}{E}\textcolor{red}{P\ }\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{T}\textcolor{red}{I}\textcolor{red}{L}\textcolor{green}{V}\textcolor{red}{V\ }\textcolor{red}{R}\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{Q}\textcolor{red}{V}\textcolor{green}{Q}\textcolor{red}{F}\textcolor{black}{K}\textcolor{green}{W}\textcolor{red}{S\ }\textcolor{green}{F}\textcolor{red}{D}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{N\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{P\ }\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{D}\textcolor{black}{K\ }\\
\\
\textcolor{green}{F}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{F}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A2Z2J8L1.tex <==


ID = A0A2Z2J8L1



Description = Bacterial leucyl aminopeptidase n=5 Tax=Escherichia coli TaxID=562 RepID=A0A2Z2J8L1\_ECOLX

Length = 292 (aa)

Predicted matches = 209 / 254 (82.28\%)

TM-score = 0.9653

Superposition in the TM-score: Length(d<5.0)= 285

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A2Z2J8L1.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{T}\textcolor{red}{F}\textcolor{red}{T}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{F}\textcolor{red}{R}\textcolor{red}{L}\textcolor{red}{S\ }\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{T}\textcolor{red}{L}\textcolor{red}{P}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{P}\textcolor{red}{A\ }\textcolor{red}{A}\textcolor{red}{Q}\textcolor{green}{P}\textcolor{red}{P}\textcolor{red}{I}\textcolor{red}{T}\textcolor{green}{D}\textcolor{red}{H}\textcolor{red}{V}\textcolor{red}{A\ }\textcolor{red}{D}\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{R}\textcolor{red}{Q}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{black}{K\ }\textcolor{green}{E}\textcolor{red}{R}\textcolor{green}{F}\textcolor{red}{I}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{R}\textcolor{red}{V\ }\textcolor{red}{R}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G\ }\textcolor{red}{Q}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{G\ }\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{red}{H}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{E\ }\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{H}\textcolor{red}{A}\textcolor{red}{N}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{Q}\textcolor{red}{L\ }\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{T}\textcolor{red}{V}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{red}{T}\textcolor{red}{Q}\textcolor{red}{T\ }\textcolor{red}{V}\textcolor{red}{H}\textcolor{green}{P}\textcolor{red}{R}\textcolor{red}{S}\textcolor{red}{A}\textcolor{green}{D}\textcolor{red}{N}\textcolor{red}{I}\textcolor{red}{D\ }\textcolor{red}{N}\textcolor{green}{L}\textcolor{red}{N}\textcolor{green}{R}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{black}{K\ }\textcolor{green}{E}\textcolor{red}{V}\textcolor{green}{F}\textcolor{red}{V}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{R}\textcolor{red}{I\ }\textcolor{red}{T}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G\ }\textcolor{red}{P}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{G\ }\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{I}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{E\ }\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L\ }\\
\\
\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{P}\textcolor{red}{H}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{R\ }\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{D\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{black}{Y\ }\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{red}{D}\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{M\ }\textcolor{red}{D}\textcolor{red}{T}\textcolor{red}{F}\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{black}{K\ }\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{S\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{P}\textcolor{red}{P}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{R\ }\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{D\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{black}{Y\ }\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{M\ }\textcolor{red}{Q}\textcolor{red}{D}\textcolor{red}{I}\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{black}{K\ }\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{S\ }\\
\\
\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{black}{K\ }\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{N\ }\textcolor{red}{F}\textcolor{black}{K}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{black}{K\ }\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{N\ }\textcolor{red}{S}\textcolor{black}{K}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A376YHF5.tex <==


ID = A0A376YHF5



Description = Anaerobic ribonucleoside-triphosphate reductase-activating protein n=1 Tax=Escherichia coli TaxID=562 RepID=A0A376YHF5\_ECOLX

Length = 139 (aa)

Predicted matches = 98 / 118 (83.05\%)

TM-score = 0.9108

Superposition in the TM-score: Length(d<5.0)= 130

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A376YHF5.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{E}\textcolor{black}{C\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{R\ }\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{T}\textcolor{black}{K}\textcolor{red}{P\ }\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{red}{R}\textcolor{green}{S\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{Q\ }\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{red}{A}\textcolor{red}{Q}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{D\ }\textcolor{red}{R}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{E}\textcolor{black}{C\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{R\ }\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{T}\textcolor{black}{K}\textcolor{red}{A\ }\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{S\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{Q\ }\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{red}{I}\textcolor{red}{L}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{D\ }\textcolor{red}{I}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D\ }\\
\\
\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{red}{R}\textcolor{red}{R}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{D}\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{D}\textcolor{red}{T}\textcolor{black}{K\ }\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{L}\textcolor{red}{F}\textcolor{black}{K}\textcolor{red}{N}\textcolor{red}{Q}\textcolor{red}{E}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{I}\textcolor{red}{N}\textcolor{red}{V}\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{D}\textcolor{red}{G}\textcolor{black}{K\ }\textcolor{red}{F}\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{D}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{P}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A377BLE3.tex <==


ID = A0A377BLE3



Description = Putative decarboxylase n=7 Tax=Escherichia coli TaxID=562 RepID=A0A377BLE3\_ECOLX

Length = 185 (aa)

Predicted matches = 142 / 167 (85.03\%)

TM-score = 0.6841

Superposition in the TM-score: Length(d<5.0)= 126

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A377BLE3.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{red}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{H\ }\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{P\ }\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{W}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{I\ }\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{W\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{black}{C}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{F}\textcolor{black}{C}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{S}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{H\ }\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{P\ }\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{W}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{I\ }\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{W\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{black}{C}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{F}\textcolor{black}{C}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{S}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S\ }\\
\\
\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{H}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{L\ }\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{green}{L}\textcolor{red}{A\ }\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{F}\textcolor{red}{A}\textcolor{red}{R}\textcolor{red}{L}\textcolor{black}{M}\textcolor{red}{A}\textcolor{red}{H}\textcolor{green}{P\ }\textcolor{red}{Q}\textcolor{red}{G}\textcolor{red}{A}\textcolor{black}{C}\textcolor{red}{G}\textcolor{red}{I}\textcolor{red}{P}\textcolor{red}{E}\textcolor{black}{K}\textcolor{red}{Q\ }\textcolor{red}{L}\textcolor{red}{H}\textcolor{black}{K}\textcolor{red}{D}\textcolor{red}{S}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{L\ }\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{red}{N}\textcolor{green}{L}\textcolor{red}{S\ }\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{F}\textcolor{red}{N}\textcolor{red}{S}\textcolor{red}{A}\textcolor{black}{M}\textcolor{red}{D}\textcolor{red}{I}\textcolor{green}{P\ }\textcolor{red}{L}\textcolor{red}{R}\textcolor{red}{G}\textcolor{black}{C}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{F}\textcolor{red}{R}\textcolor{black}{K}\textcolor{red}{N\ }\textcolor{red}{V}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{R}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A377CTF9.tex <==


ID = A0A377CTF9



Description = tRNA-specific adenosine deaminase n=1 Tax=Escherichia coli TaxID=562 RepID=A0A377CTF9\_ECOLX

Length = 167 (aa)

Predicted matches = 122 / 147 (82.99\%)

TM-score = 0.9577

Superposition in the TM-score: Length(d<5.0)= 161

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A377CTF9.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{S}\textcolor{red}{W}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{E}\textcolor{green}{S}\textcolor{red}{Q}\textcolor{red}{I}\textcolor{black}{Y\ }\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{R}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{R}\textcolor{red}{I}\textcolor{red}{S}\textcolor{red}{E}\textcolor{black}{K\ }\textcolor{red}{L}\textcolor{red}{G}\textcolor{green}{W}\textcolor{red}{N}\textcolor{green}{E}\textcolor{red}{W}\textcolor{green}{E}\textcolor{red}{W}\textcolor{green}{P}\textcolor{red}{A\ }\textcolor{green}{G}\textcolor{red}{V}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{H}\textcolor{green}{N}\textcolor{red}{V}\textcolor{green}{R}\textcolor{green}{V\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{E}\textcolor{red}{W}\textcolor{green}{W}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{red}{A}\textcolor{red}{D}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{I\ }\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{V}\textcolor{black}{M}\textcolor{black}{C\ }\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{K\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{S}\textcolor{red}{E}\textcolor{red}{V}\textcolor{red}{E}\textcolor{red}{F}\textcolor{green}{S}\textcolor{red}{H}\textcolor{red}{E}\textcolor{black}{Y\ }\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{R}\textcolor{red}{H}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{A}\textcolor{black}{K\ }\textcolor{red}{R}\textcolor{red}{A}\textcolor{green}{W}\textcolor{red}{D}\textcolor{green}{E}\textcolor{red}{R}\textcolor{green}{E}\textcolor{red}{V}\textcolor{green}{P}\textcolor{red}{V\ }\textcolor{green}{G}\textcolor{red}{A}\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{H}\textcolor{green}{N}\textcolor{red}{N}\textcolor{green}{R}\textcolor{green}{V\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{E}\textcolor{red}{G}\textcolor{green}{W}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{red}{R}\textcolor{red}{H}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{I\ }\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{V}\textcolor{black}{M}\textcolor{black}{C\ }\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{K\ }\\
\\
\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{D}\textcolor{red}{V\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E\ }\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{R\ }\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{D}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{D}\textcolor{red}{L\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E\ }\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{R\ }\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{D}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A377CY91.tex <==


ID = A0A377CY91



Description = Outer membrane protein F n=1 Tax=Escherichia coli TaxID=562 RepID=A0A377CY91\_ECOLX

Length = 280 (aa)

Predicted matches = 181 / 239 (75.73\%)

TM-score = 0.9363

Superposition in the TM-score: Length(d<5.0)= 268

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A377CY91.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{R}\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{M\ }\textcolor{red}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{red}{D}\textcolor{green}{S}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{N\ }\textcolor{green}{N}\textcolor{red}{L}\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{red}{N}\textcolor{red}{D\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{R}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{M\ }\textcolor{red}{T}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{red}{N}\textcolor{green}{S}\textcolor{red}{D}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{N\ }\textcolor{green}{N}\textcolor{red}{S}\textcolor{green}{E}\textcolor{red}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{red}{T}\textcolor{red}{G\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L\ }\\
\\
\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{F\ }\textcolor{red}{N}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{D}\textcolor{red}{S}\textcolor{green}{F\ }\textcolor{green}{F}\textcolor{red}{D}\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{F}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{A}\textcolor{red}{V}\textcolor{red}{E\ }\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{G}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{black}{Y}\textcolor{red}{N}\textcolor{black}{Y}\textcolor{red}{R}\textcolor{red}{D}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{G}\textcolor{red}{V}\textcolor{black}{Y}\textcolor{red}{T}\textcolor{red}{E}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{N\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{F\ }\textcolor{red}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{F\ }\textcolor{green}{F}\textcolor{red}{V}\textcolor{red}{G}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{G}\textcolor{red}{G}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{F}\textcolor{red}{F}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{D}\textcolor{red}{T}\textcolor{green}{A}\textcolor{red}{R}\textcolor{red}{R\ }\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{black}{Y}\textcolor{red}{E}\textcolor{black}{Y}\textcolor{red}{E}\textcolor{red}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{G}\textcolor{red}{A}\textcolor{black}{Y}\textcolor{red}{G}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{N\ }\\
\\
\textcolor{red}{A}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{red}{E}\textcolor{red}{N}\textcolor{red}{T}\textcolor{red}{R}\textcolor{red}{A}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{N}\textcolor{red}{D}\textcolor{red}{N}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{A}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{N}\textcolor{red}{V}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{red}{A}\textcolor{black}{Y}\textcolor{red}{N}\textcolor{green}{E}\textcolor{red}{N}\textcolor{green}{R}\textcolor{red}{T}\textcolor{red}{G}\textcolor{red}{D\ }\textcolor{red}{W}\textcolor{red}{G}\textcolor{green}{T}\textcolor{red}{R}\textcolor{black}{K}\textcolor{red}{N}\textcolor{red}{D}\textcolor{red}{S}\textcolor{red}{G}\textcolor{red}{T\ }\textcolor{red}{E}\textcolor{red}{D}\textcolor{green}{P}\textcolor{red}{I}\textcolor{black}{K}\textcolor{red}{N}\textcolor{black}{K}\textcolor{red}{D}\textcolor{red}{T}\textcolor{black}{C\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{red}{L}\textcolor{green}{Q}\textcolor{red}{E}\textcolor{red}{A}\textcolor{red}{Q}\textcolor{red}{P}\textcolor{red}{L}\textcolor{red}{G}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{E}\textcolor{red}{Q}\textcolor{red}{W}\textcolor{green}{A}\textcolor{red}{T}\textcolor{red}{G}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{N}\textcolor{red}{N}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{red}{N}\textcolor{black}{Y}\textcolor{red}{G}\textcolor{green}{E}\textcolor{red}{T}\textcolor{green}{R}\textcolor{red}{N}\textcolor{red}{A}\textcolor{red}{T\ }\textcolor{red}{P}\textcolor{red}{I}\textcolor{green}{T}\textcolor{red}{N}\textcolor{black}{K}\textcolor{red}{F}\textcolor{red}{T}\textcolor{red}{T}\textcolor{red}{S}\textcolor{red}{A\ }\textcolor{red}{A}\textcolor{red}{S}\textcolor{green}{P}\textcolor{red}{T}\textcolor{black}{K}\textcolor{red}{R}\textcolor{black}{K}\textcolor{red}{T}\textcolor{red}{F}\textcolor{black}{C\ }\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A377D2A6.tex <==


ID = A0A377D2A6



Description = Protein n=1 Tax=Escherichia coli TaxID=562 RepID=A0A377D2A6\_ECOLX

Length = 209 (aa)

Predicted matches = 147 / 172 (85.47\%)

TM-score = 0.707

Superposition in the TM-score: Length(d<5.0)= 155

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A377D2A6.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{V\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{W\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{Q\ }\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{V\ }\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{E}\textcolor{red}{S}\textcolor{green}{G\ }\textcolor{green}{D}\textcolor{red}{V}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{L}\textcolor{red}{P}\textcolor{red}{E\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{G}\textcolor{green}{Q}\textcolor{black}{Y\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{V\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{W\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{Q\ }\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{V\ }\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{F}\textcolor{red}{H}\textcolor{green}{G\ }\textcolor{green}{D}\textcolor{red}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{L}\textcolor{red}{T}\textcolor{red}{N\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{Q}\textcolor{black}{Y\ }\\
\\
\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{E}\textcolor{black}{K}\textcolor{black}{M\ }\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{G}\textcolor{red}{D}\textcolor{black}{M\ }\textcolor{green}{E}\textcolor{red}{Q}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{A\ }\textcolor{red}{R}\textcolor{red}{S}\textcolor{red}{E}\textcolor{red}{I}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{E}\textcolor{black}{K}\textcolor{black}{M}\textcolor{red}{Q\ }\textcolor{red}{A}\textcolor{red}{E}\textcolor{green}{S}\textcolor{red}{W}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{I}\textcolor{black}{C}\textcolor{red}{Q}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{E}\textcolor{black}{K}\textcolor{black}{M\ }\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{red}{V}\textcolor{green}{G}\textcolor{red}{V}\textcolor{black}{M\ }\textcolor{green}{E}\textcolor{red}{N}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{P}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{A\ }\textcolor{red}{T}\textcolor{red}{W}\textcolor{red}{R}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{V}\textcolor{red}{R}\textcolor{black}{K}\textcolor{black}{M}\textcolor{red}{E\ }\textcolor{red}{S}\textcolor{red}{S}\textcolor{green}{S}\textcolor{red}{I}\textcolor{red}{A}\textcolor{black}{K}\textcolor{red}{H}\textcolor{black}{C}\textcolor{red}{L}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A377KE78.tex <==


ID = A0A377KE78



Description = Vitamin B12-binding protein n=3 Tax=Escherichia coli TaxID=562 RepID=A0A377KE78\_ECOLX

Length = 266 (aa)

Predicted matches = 182 / 240 (75.83\%)

TM-score = 0.8598

Superposition in the TM-score: Length(d<5.0)= 232

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A377KE78.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{A}\textcolor{black}{K}\textcolor{red}{F}\textcolor{green}{L}\textcolor{green}{F}\textcolor{red}{F}\textcolor{red}{I}\textcolor{green}{L}\textcolor{red}{T\ }\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{E}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{G}\textcolor{red}{W\ }\textcolor{black}{Y}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{F}\textcolor{red}{E}\textcolor{red}{S}\textcolor{red}{P}\textcolor{red}{E\ }\textcolor{red}{L}\textcolor{red}{I}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{G\ }\textcolor{red}{A}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{red}{N}\textcolor{green}{T}\textcolor{red}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{N\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{T\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{A}\textcolor{black}{K}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{F}\textcolor{red}{R}\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{V\ }\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{F}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{L}\textcolor{red}{W}\textcolor{red}{L\ }\textcolor{black}{Y}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{I}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{S\ }\textcolor{red}{P}\textcolor{red}{A}\textcolor{red}{N}\textcolor{red}{T}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{F}\textcolor{red}{A}\textcolor{red}{A\ }\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{red}{S}\textcolor{green}{T}\textcolor{red}{W}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{N\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{T\ }\\
\\
\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{D}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{L\ }\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{V}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{red}{E\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{P}\textcolor{red}{P}\textcolor{green}{Q}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{red}{A}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{red}{E}\textcolor{red}{E}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{Y\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{red}{P}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{V}\textcolor{red}{G}\textcolor{green}{L\ }\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{red}{D}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{F}\textcolor{black}{K\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{S\ }\textcolor{green}{R}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{R}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{D}\textcolor{red}{L\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{red}{S}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{N}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{R\ }\textcolor{red}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{W}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{red}{D\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{red}{E}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{red}{D}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{red}{Q}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{Y\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{red}{S}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{L\ }\textcolor{red}{Q}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{red}{N}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{F}\textcolor{black}{K\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{S\ }\textcolor{green}{R}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{R}\textcolor{red}{S}\textcolor{green}{P}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{P}\textcolor{green}{D}\textcolor{red}{Q\ }\\
\\
\textcolor{green}{I}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{D}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{I}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{P}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{D}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A377N083.tex <==


ID = A0A377N083



Description = Endolysin n=1 Tax=Escherichia coli TaxID=562 RepID=A0A377N083\_ECOLX

Length = 204 (aa)

Predicted matches = 144 / 182 (79.12\%)

TM-score = 0.9195

Superposition in the TM-score: Length(d<5.0)= 189

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A377N083.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{red}{W}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{V}\textcolor{red}{A}\textcolor{green}{R}\textcolor{green}{W\ }\textcolor{green}{F}\textcolor{red}{A}\textcolor{red}{H}\textcolor{red}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{green}{F}\textcolor{red}{Q}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{Q}\textcolor{red}{T}\textcolor{red}{R}\textcolor{green}{E}\textcolor{red}{D\ }\textcolor{red}{D}\textcolor{green}{G}\textcolor{red}{L}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{G}\textcolor{red}{V}\textcolor{red}{R}\textcolor{green}{L\ }\textcolor{green}{N}\textcolor{black}{Y}\textcolor{red}{F}\textcolor{red}{F}\textcolor{red}{D}\textcolor{green}{A}\textcolor{red}{D}\textcolor{red}{E}\textcolor{red}{P}\textcolor{red}{S\ }\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R}\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{red}{L\ }\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{L}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{V}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{N}\textcolor{red}{E}\textcolor{red}{F\ }\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{P\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{V}\textcolor{green}{R}\textcolor{green}{W\ }\textcolor{green}{F}\textcolor{red}{Q}\textcolor{red}{P}\textcolor{red}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{red}{Q}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{green}{F}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{red}{V}\textcolor{red}{G}\textcolor{red}{H}\textcolor{green}{E}\textcolor{red}{S\ }\textcolor{red}{G}\textcolor{green}{G}\textcolor{red}{F}\textcolor{red}{S}\textcolor{green}{A}\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{E}\textcolor{red}{N}\textcolor{green}{L\ }\textcolor{green}{N}\textcolor{black}{Y}\textcolor{red}{T}\textcolor{red}{P}\textcolor{red}{S}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{V}\textcolor{red}{A}\textcolor{red}{T\ }\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R}\textcolor{red}{I}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{red}{A\ }\textcolor{red}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{R}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{H}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{N}\textcolor{red}{L}\textcolor{red}{V\ }\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{P\ }\\
\\
\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{W}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{H}\textcolor{green}{N}\textcolor{black}{Y\ }\textcolor{green}{R}\textcolor{red}{I}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{W\ }\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{black}{C}\textcolor{black}{M}\textcolor{red}{V}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{W}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{N}\textcolor{black}{Y\ }\textcolor{green}{R}\textcolor{red}{T}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{W\ }\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{black}{C}\textcolor{black}{M}\textcolor{red}{I}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A3A6T7V2.tex <==


ID = A0A3A6T7V2



Description = (Fe-S)-binding protein n=2 Tax=Escherichia coli TaxID=562 RepID=A0A3A6T7V2\_ECOLX

Length = 239 (aa)

Predicted matches = 180 / 201 (89.55\%)

TM-score = 0.9812

Superposition in the TM-score: Length(d<5.0)= 238

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A3A6T7V2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{I\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{black}{Y}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{M}\textcolor{black}{K\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{black}{C\ }\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{T}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{D\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{I\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{black}{Y}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{M}\textcolor{black}{K\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{S}\textcolor{black}{C\ }\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{T}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{red}{P}\textcolor{green}{E}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{D\ }\\
\\
\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{S}\textcolor{red}{A}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{T}\textcolor{red}{L}\textcolor{green}{H}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{E}\textcolor{red}{G\ }\textcolor{red}{V}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{E}\textcolor{red}{T}\textcolor{red}{D}\textcolor{red}{D}\textcolor{red}{G}\textcolor{red}{N}\textcolor{red}{A\ }\textcolor{red}{V}\textcolor{black}{C}\textcolor{red}{E}\textcolor{red}{T}\textcolor{green}{N}\textcolor{green}{I}\textcolor{red}{R}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{L\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{S}\textcolor{red}{G}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{V}\textcolor{red}{A}\textcolor{green}{H}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{E}\textcolor{red}{V\ }\textcolor{red}{R}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{F}\textcolor{red}{L}\textcolor{red}{I}\textcolor{red}{G}\textcolor{red}{A}\textcolor{red}{D}\textcolor{red}{V\ }\textcolor{red}{S}\textcolor{black}{C}\textcolor{red}{L}\textcolor{red}{L}\textcolor{green}{N}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{L\ }\\
\\
\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{R}\textcolor{green}{R}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{S}\textcolor{green}{R}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A3K0JUW2.tex <==


ID = A0A3K0JUW2



Description = L-lysine exporter LysO n=1 Tax=Escherichia coli TaxID=562 RepID=A0A3K0JUW2\_ECOLX

Length = 299 (aa)

Predicted matches = 214 / 275 (77.82\%)

TM-score = 0.971

Superposition in the TM-score: Length(d<5.0)= 299

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A3K0JUW2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{A\ }\textcolor{green}{P}\textcolor{red}{I}\textcolor{red}{L}\textcolor{red}{G}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{red}{Q}\textcolor{red}{V}\textcolor{red}{I}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N\ }\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{S}\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{red}{W}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{F}\textcolor{black}{M}\textcolor{red}{S}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{L\ }\textcolor{red}{S}\textcolor{green}{D}\textcolor{green}{N}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{S}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{V}\textcolor{red}{E}\textcolor{red}{R}\textcolor{green}{I}\textcolor{red}{Q\ }\textcolor{red}{G}\textcolor{green}{I}\textcolor{red}{I}\textcolor{green}{L}\textcolor{black}{C}\textcolor{red}{H}\textcolor{red}{H}\textcolor{green}{A}\textcolor{red}{T}\textcolor{red}{A\ }\textcolor{black}{M}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{A}\textcolor{black}{C}\textcolor{red}{T}\textcolor{green}{P}\textcolor{red}{L}\textcolor{red}{E\ }\textcolor{red}{V}\textcolor{red}{D}\textcolor{red}{G}\textcolor{red}{E}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{E}\textcolor{green}{P}\textcolor{red}{R\ }\textcolor{green}{R}\textcolor{green}{I}\textcolor{red}{R}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{V\ }\textcolor{green}{P}\textcolor{red}{L}\textcolor{red}{I}\textcolor{red}{V}\textcolor{red}{G}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N\ }\textcolor{red}{Q}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{F}\textcolor{black}{M}\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{F\ }\textcolor{red}{L}\textcolor{green}{D}\textcolor{green}{N}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{red}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{I}\textcolor{red}{T\ }\textcolor{red}{V}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{L}\textcolor{black}{C}\textcolor{red}{N}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{L\ }\textcolor{black}{M}\textcolor{red}{W}\textcolor{green}{L}\textcolor{red}{E}\textcolor{red}{R}\textcolor{black}{C}\textcolor{red}{L}\textcolor{green}{P}\textcolor{red}{W}\textcolor{red}{R\ }\textcolor{red}{N}\textcolor{red}{H}\textcolor{red}{H}\textcolor{red}{Q}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{L}\textcolor{green}{P}\textcolor{red}{S\ }\textcolor{green}{R}\textcolor{green}{I}\textcolor{red}{A}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{K\ }\\
\\
\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{V}\textcolor{red}{A}\textcolor{red}{F}\textcolor{green}{Q\ }\textcolor{red}{T}\textcolor{green}{A}\textcolor{red}{D}\textcolor{green}{E}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{red}{I}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{red}{I\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{red}{S}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{Q\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{red}{P}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{A\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{P}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{G}\textcolor{red}{G}\textcolor{green}{V\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{F}\textcolor{red}{L}\textcolor{green}{Q\ }\textcolor{red}{H}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{A}\textcolor{red}{S}\textcolor{red}{E}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{red}{L\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{Q\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q\ }\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{A\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{G}\textcolor{red}{P}\textcolor{green}{V\ }\\
\\
\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{T\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{G}\textcolor{black}{M\ }\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{T}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{R}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I\ }\textcolor{red}{R}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{F}\textcolor{green}{S}\textcolor{red}{L}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{T\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{S}\textcolor{black}{M\ }\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{T}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{green}{R}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I\ }\textcolor{red}{V}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{A}\textcolor{red}{F}\textcolor{green}{F}\textcolor{green}{S}\textcolor{red}{A}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A3Q0N3K2.tex <==


ID = A0A3Q0N3K2



Description = ArsR family transcriptional regulator n=3 Tax=Enterobacteriaceae TaxID=543 RepID=A0A3Q0N3K2\_ECOLX

Length = 107 (aa)

Predicted matches = 79 / 94 (84.04\%)

TM-score = 0.8811

Superposition in the TM-score: Length(d<5.0)= 97

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A3Q0N3K2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{G}\textcolor{red}{R}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{green}{I}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{Q}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{V}\textcolor{red}{D}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{Q}\textcolor{red}{E}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{S\ }\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{E}\textcolor{red}{F}\textcolor{green}{R}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{red}{P}\textcolor{green}{I}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{I}\textcolor{red}{D}\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{W}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{K}\textcolor{red}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{red}{A\ }\textcolor{green}{E}\textcolor{red}{H}\textcolor{red}{R}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{G}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{G}\textcolor{red}{H}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{green}{I}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{Q}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{V}\textcolor{red}{G}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{Q}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{S\ }\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{red}{E}\textcolor{green}{I}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{I}\textcolor{red}{E}\textcolor{red}{F}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{D}\textcolor{green}{V}\textcolor{red}{T\ }\textcolor{green}{E}\textcolor{red}{P}\textcolor{red}{A}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{G}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A5B9AN37.tex <==


ID = A0A5B9AN37



Description = HTH-type transcriptional activator RhaS n=1 Tax=Escherichia coli TaxID=562 RepID=A0A5B9AN37\_ECOLX

Length = 278 (aa)

Predicted matches = 233 / 261 (89.27\%)

TM-score = 0.8827

Superposition in the TM-score: Length(d<5.0)= 250

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A5B9AN37.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{E\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{E\ }\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{H}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{black}{C\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{Q\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{Y\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{E\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{E\ }\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{H}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{black}{C\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{Q\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{Y\ }\\
\\
\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{Q\ }\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{red}{G}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{N}\textcolor{red}{L}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{red}{H}\textcolor{green}{H}\textcolor{green}{F}\textcolor{red}{D}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{N}\textcolor{red}{E\ }\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{V}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{red}{V}\textcolor{red}{G}\textcolor{green}{L}\textcolor{red}{L\ }\textcolor{red}{E}\textcolor{red}{S}\textcolor{red}{D}\textcolor{red}{T}\textcolor{green}{H}\textcolor{red}{G}\textcolor{red}{S}\textcolor{red}{R}\textcolor{black}{K}\textcolor{red}{R\ }\textcolor{black}{K}\textcolor{red}{P}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{T}\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{W}\textcolor{black}{Y}\textcolor{red}{W\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{Q\ }\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{N}\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{W}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{red}{D}\textcolor{green}{H}\textcolor{green}{F}\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{N}\textcolor{red}{W\ }\textcolor{green}{D}\textcolor{red}{A}\textcolor{green}{V}\textcolor{green}{A}\textcolor{red}{D}\textcolor{green}{Q}\textcolor{red}{F}\textcolor{red}{S}\textcolor{green}{L}\textcolor{red}{S\ }\textcolor{red}{L}\textcolor{red}{R}\textcolor{red}{T}\textcolor{red}{L}\textcolor{green}{H}\textcolor{red}{R}\textcolor{red}{Q}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{Q\ }\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{G}\textcolor{red}{L}\textcolor{green}{T}\textcolor{red}{P}\textcolor{red}{Q}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{red}{L\ }\\
\\
\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{T\ }\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{G}\textcolor{red}{V}\textcolor{green}{S}\textcolor{green}{D\ }\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{W}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{R}\textcolor{red}{R}\textcolor{green}{I}\textcolor{green}{R\ }\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{Q}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{red}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{T\ }\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{G}\textcolor{red}{F}\textcolor{green}{S}\textcolor{green}{D\ }\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{W}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{R}\textcolor{red}{D}\textcolor{green}{I}\textcolor{green}{R\ }\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{Q}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A5B9B0Y2.tex <==


ID = A0A5B9B0Y2



Description = MFS transporter n=1 Tax=Escherichia coli TaxID=562 RepID=A0A5B9B0Y2\_ECOLX

Length = 417 (aa)

Predicted matches = 325 / 375 (86.67\%)

TM-score = 0.9467

Superposition in the TM-score: Length(d<5.0)= 388

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A5B9B0Y2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{L}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{P}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L\ }\\
\\
\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{T}\textcolor{black}{M\ }\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{I}\textcolor{red}{P}\textcolor{red}{V}\textcolor{black}{M\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{F\ }\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{S\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{R}\textcolor{red}{A}\textcolor{red}{R}\textcolor{green}{S\ }\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{F}\textcolor{green}{T}\textcolor{red}{R}\textcolor{green}{F}\textcolor{green}{F}\textcolor{red}{I}\textcolor{green}{W}\textcolor{red}{A\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{F}\textcolor{red}{R\ }\textcolor{green}{L}\textcolor{red}{P}\textcolor{red}{T}\textcolor{red}{G}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{S}\textcolor{green}{W}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{I}\textcolor{red}{P}\textcolor{red}{G}\textcolor{red}{D}\textcolor{red}{V}\textcolor{red}{S}\textcolor{red}{G}\textcolor{red}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{T}\textcolor{black}{M\ }\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{I}\textcolor{red}{L}\textcolor{red}{I}\textcolor{black}{M\ }\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{F\ }\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{S\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{R}\textcolor{red}{L}\textcolor{red}{I}\textcolor{green}{S\ }\textcolor{green}{G}\textcolor{red}{V}\textcolor{green}{F}\textcolor{green}{T}\textcolor{red}{D}\textcolor{green}{F}\textcolor{green}{F}\textcolor{red}{N}\textcolor{green}{W}\textcolor{red}{R\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{F}\textcolor{red}{A\ }\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{A}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{F}\textcolor{green}{W}\textcolor{black}{K}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{S}\textcolor{red}{R}\textcolor{red}{H}\textcolor{red}{F}\textcolor{red}{R}\textcolor{red}{P}\textcolor{red}{T\ }\\
\\
\textcolor{red}{R}\textcolor{red}{A}\textcolor{black}{C}\textcolor{red}{G}\textcolor{black}{K}\textcolor{red}{P}\textcolor{green}{L}\textcolor{red}{D}\textcolor{red}{A}\textcolor{green}{N\ }\textcolor{red}{R}\textcolor{red}{I}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{red}{S}\textcolor{red}{S}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{L}\textcolor{red}{T\ }\textcolor{red}{L}\textcolor{red}{S}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{F}\textcolor{red}{A}\textcolor{red}{A\ }\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{N}\textcolor{black}{Y\ }\textcolor{red}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{red}{F}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{W\ }\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{R\ }\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{F\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{red}{S}\textcolor{red}{L}\textcolor{black}{C}\textcolor{red}{P}\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{L}\textcolor{red}{F}\textcolor{red}{I}\textcolor{green}{N\ }\textcolor{red}{F}\textcolor{red}{R}\textcolor{green}{L}\textcolor{red}{H}\textcolor{red}{W}\textcolor{red}{R}\textcolor{red}{D}\textcolor{red}{R}\textcolor{red}{G}\textcolor{red}{L\ }\textcolor{red}{P}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{A}\textcolor{red}{E}\textcolor{green}{G}\textcolor{green}{F}\textcolor{red}{L}\textcolor{red}{L\ }\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{N}\textcolor{black}{Y\ }\textcolor{red}{I}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{red}{L}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{R\ }\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{W}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{R\ }\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{F\ }\\
\\
\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{W\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{G\ }\textcolor{red}{Q}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{W\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{A}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{W\ }\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{G\ }\textcolor{red}{R}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{W\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{M\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{A}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A6N3ILI5.tex <==


ID = A0A6N3ILI5



Description = IS6 family transposase n=1 Tax=Escherichia coli TaxID=562 RepID=A0A6N3ILI5\_ECOLX

Length = 192 (aa)

Predicted matches = 110 / 154 (71.43\%)

TM-score = 0.4524

Superposition in the TM-score: Length(d<5.0)= 93

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A6N3ILI5.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{G}\textcolor{red}{L}\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{Q\ }\textcolor{red}{H}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{W\ }\textcolor{black}{Y}\textcolor{black}{C}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{E\ }\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{E}\textcolor{red}{N}\textcolor{green}{G}\textcolor{red}{T\ }\textcolor{green}{N}\textcolor{red}{E}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{T}\textcolor{red}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{red}{L\ }\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{P}\textcolor{black}{Y}\textcolor{red}{V}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{M}\textcolor{red}{R}\textcolor{black}{K\ }\textcolor{red}{E}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{red}{Q}\textcolor{red}{D}\textcolor{red}{A}\textcolor{red}{E\ }\textcolor{red}{G}\textcolor{red}{G}\textcolor{black}{C}\textcolor{red}{W}\textcolor{red}{L}\textcolor{red}{V}\textcolor{black}{M}\textcolor{red}{N}\textcolor{black}{K}\textcolor{red}{L\ }\textcolor{green}{L}\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{F}\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{V}\textcolor{green}{I}\textcolor{red}{Q\ }\textcolor{green}{R}\textcolor{red}{E}\textcolor{red}{R}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{A}\textcolor{red}{D}\textcolor{red}{T\ }\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{D}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{R\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{G}\textcolor{red}{R}\textcolor{green}{H}\textcolor{green}{F}\textcolor{green}{Q\ }\textcolor{red}{R}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{W\ }\textcolor{black}{Y}\textcolor{black}{C}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{E\ }\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{E}\textcolor{red}{R}\textcolor{green}{G}\textcolor{red}{V\ }\textcolor{green}{N}\textcolor{red}{V}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{T}\textcolor{red}{I}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{red}{W\ }\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{E}\textcolor{black}{M}\textcolor{red}{E}\textcolor{black}{K\ }\textcolor{red}{R}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{red}{W}\textcolor{red}{R}\textcolor{red}{N}\textcolor{red}{P}\textcolor{red}{S\ }\textcolor{red}{D}\textcolor{red}{L}\textcolor{black}{C}\textcolor{red}{P}\textcolor{red}{W}\textcolor{red}{H}\textcolor{black}{M}\textcolor{red}{G}\textcolor{black}{K}\textcolor{red}{I\ }\textcolor{green}{L}\textcolor{red}{N}\textcolor{red}{N}\textcolor{red}{V}\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{W}\textcolor{red}{Q}\textcolor{green}{I}\textcolor{red}{P\ }\textcolor{green}{R}\textcolor{red}{F}\textcolor{red}{I}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{A\ }\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{R}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{R\ }\\
\\
\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{E}\textcolor{red}{G\ }\textcolor{green}{R}\textcolor{red}{N}\textcolor{green}{I}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{I}\textcolor{red}{G}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{S}\textcolor{black}{M\ }\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{E}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{red}{P}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{black}{M}\\
\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\\
\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{E}\textcolor{red}{H\ }\textcolor{green}{R}\textcolor{red}{Q}\textcolor{green}{I}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{green}{I}\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{S}\textcolor{black}{M\ }\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{I}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{Q\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{black}{M}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A765X5V4.tex <==


ID = A0A765X5V4



Description = Carboxy-S-adenosyl-L-methionine synthase n=2 Tax=Escherichia TaxID=561 RepID=A0A765X5V4\_ECOLX

Length = 247 (aa)

Predicted matches = 180 / 219 (82.19\%)

TM-score = 0.9728

Superposition in the TM-score: Length(d<5.0)= 245

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A765X5V4.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{F\ }\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{S\ }\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{H\ }\textcolor{green}{D}\textcolor{green}{N}\textcolor{black}{C}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{N\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{R}\textcolor{red}{H\ }\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{P\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{F\ }\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{S\ }\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{H\ }\textcolor{green}{D}\textcolor{green}{N}\textcolor{black}{C}\textcolor{black}{K}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{N\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{I}\textcolor{red}{E}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{R}\textcolor{red}{R\ }\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{P\ }\\
\\
\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{D\ }\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{P\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{K}\textcolor{red}{L\ }\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{N}\textcolor{black}{M\ }\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{W}\textcolor{green}{E}\textcolor{green}{I}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{S\ }\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{N}\textcolor{red}{L}\textcolor{black}{M}\textcolor{red}{P}\textcolor{red}{A}\textcolor{red}{E}\textcolor{red}{F\ }\textcolor{red}{F}\textcolor{red}{L}\textcolor{red}{E}\textcolor{red}{I}\textcolor{black}{K}\textcolor{red}{F}\textcolor{red}{A}\textcolor{red}{R}\textcolor{red}{G}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{D\ }\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{P\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{red}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{K}\textcolor{red}{I\ }\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{N}\textcolor{black}{M\ }\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{L}\textcolor{green}{E}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{S\ }\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{N}\textcolor{red}{V}\textcolor{black}{M}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{D}\textcolor{red}{S\ }\textcolor{red}{V}\textcolor{red}{E}\textcolor{red}{T}\textcolor{red}{H}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{R}\textcolor{red}{L}\textcolor{red}{H}\textcolor{black}{K\ }\\
\\
\textcolor{red}{L}\textcolor{red}{R}\textcolor{red}{D}\textcolor{red}{G}\textcolor{red}{R}\textcolor{red}{I}\textcolor{red}{T}\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{V\ }\textcolor{red}{T}\textcolor{black}{C}\textcolor{red}{I}\textcolor{green}{N}\textcolor{red}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{A\ }\textcolor{red}{N}\textcolor{black}{K}\textcolor{red}{E}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{red}{A}\textcolor{red}{G}\textcolor{red}{F}\textcolor{red}{E}\textcolor{red}{H}\textcolor{red}{S}\textcolor{red}{E}\textcolor{green}{L}\textcolor{red}{W}\textcolor{red}{F\ }\textcolor{red}{Q}\textcolor{black}{C}\textcolor{red}{F}\textcolor{green}{N}\textcolor{red}{F}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7A2W9Z6.tex <==


ID = A0A7A2W9Z6



Description = DUF1190 domain-containing protein n=2 Tax=Escherichia TaxID=561 RepID=A0A7A2W9Z6\_ECOLX

Length = 212 (aa)

Predicted matches = 142 / 180 (78.89\%)

TM-score = 0.5901

Superposition in the TM-score: Length(d<5.0)= 126

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7A2W9Z6.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{N}\textcolor{red}{N\ }\textcolor{red}{T}\textcolor{black}{K}\textcolor{red}{I}\textcolor{red}{G}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{red}{G}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{F}\textcolor{red}{E}\textcolor{green}{P\ }\textcolor{red}{R}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{F\ }\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{G}\textcolor{black}{C}\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{F\ }\textcolor{black}{Y}\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{black}{C}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{G\ }\textcolor{green}{W}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{A\ }\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{N}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{N\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{N}\textcolor{red}{S\ }\textcolor{red}{S}\textcolor{black}{K}\textcolor{red}{P}\textcolor{red}{A}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{red}{N}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{F}\textcolor{red}{A}\textcolor{green}{P\ }\textcolor{red}{Q}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{H}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{F\ }\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{S}\textcolor{black}{C}\textcolor{red}{G}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{D}\textcolor{red}{V}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{F\ }\textcolor{black}{Y}\textcolor{red}{S}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{black}{C}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{A}\textcolor{red}{H}\textcolor{green}{G\ }\textcolor{green}{W}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{A\ }\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{N}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{N\ }\\
\\
\textcolor{black}{C}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{E}\textcolor{red}{A}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{black}{Y\ }\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{S}\textcolor{green}{W}\textcolor{red}{I}\textcolor{green}{P}\textcolor{green}{V\ }\textcolor{red}{V}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{V}\textcolor{red}{S\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{E}\textcolor{red}{N}\textcolor{red}{G}\textcolor{red}{P}\textcolor{black}{Y\ }\textcolor{green}{N}\textcolor{red}{Q}\textcolor{green}{G}\textcolor{red}{S}\textcolor{red}{G}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{red}{N}\textcolor{red}{T}\textcolor{red}{T\ }\textcolor{red}{S}\textcolor{red}{I}\textcolor{red}{N}\textcolor{red}{D}\textcolor{red}{D}\textcolor{red}{R}\textcolor{red}{A}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{S}\textcolor{red}{E}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{S}\textcolor{red}{N}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{H}\textcolor{red}{D\ }\textcolor{green}{G}\textcolor{green}{G}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{black}{C}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{E}\textcolor{red}{N}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{black}{Y\ }\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{green}{S}\textcolor{green}{W}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{V\ }\textcolor{red}{I}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{V}\textcolor{red}{I\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{red}{F}\textcolor{red}{V}\textcolor{black}{Y\ }\textcolor{green}{N}\textcolor{red}{S}\textcolor{green}{G}\textcolor{red}{G}\textcolor{red}{S}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{R\ }\textcolor{red}{P}\textcolor{red}{V}\textcolor{red}{W}\textcolor{red}{R}\textcolor{red}{N}\textcolor{red}{T}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{S}\textcolor{red}{W}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{S}\textcolor{red}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{H}\textcolor{red}{W\ }\textcolor{green}{G}\textcolor{green}{G}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7B1S4X3.tex <==


ID = A0A7B1S4X3



Description = Terminase large subunit n=1 Tax=Escherichia coli TaxID=562 RepID=A0A7B1S4X3\_ECOLX

Length = 498 (aa)

Predicted matches = 343 / 428 (80.14\%)

TM-score = 0.6286

Superposition in the TM-score: Length(d<5.0)= 274

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7B1S4X3.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{I}\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{W}\textcolor{green}{V\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{N\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{F\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{T\ }\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{red}{N}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{red}{H}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{C}\textcolor{black}{K}\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{black}{M\ }\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{P}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{N}\textcolor{black}{M}\textcolor{red}{T}\textcolor{green}{R}\textcolor{red}{D}\textcolor{red}{L}\textcolor{green}{D}\textcolor{green}{G\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{I}\textcolor{black}{C}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{W}\textcolor{green}{V\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{N\ }\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{F\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{T\ }\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{red}{R}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{C}\textcolor{black}{K}\textcolor{red}{R}\textcolor{green}{T}\textcolor{green}{P}\textcolor{black}{M\ }\textcolor{green}{L}\textcolor{red}{T}\textcolor{red}{E}\textcolor{green}{A}\textcolor{red}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{N}\textcolor{black}{M}\textcolor{red}{N}\textcolor{green}{R}\textcolor{red}{P}\textcolor{red}{E}\textcolor{green}{D}\textcolor{green}{G\ }\\
\\
\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{H}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{M\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{L}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{G\ }\textcolor{green}{P}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{V\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{H}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{M\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{M}\textcolor{red}{W}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{G\ }\textcolor{green}{P}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{I\ }\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{V\ }\\
\\
\textcolor{green}{S}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{S}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{green}{I}\textcolor{green}{W}\textcolor{red}{Q}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{F\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{G\ }\textcolor{green}{Q}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{T\ }\textcolor{green}{H}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{W\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{E\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\\
\textcolor{green}{S}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{N\ }\textcolor{green}{I}\textcolor{green}{W}\textcolor{red}{V}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{F\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{E}\textcolor{green}{D\ }\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{G\ }\textcolor{green}{Q}\textcolor{green}{P}\textcolor{black}{C}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{T\ }\textcolor{green}{H}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{W\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{E\ }\\
\\
\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R\ }\textcolor{green}{F}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{red}{H}\textcolor{green}{T}\textcolor{red}{N}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{N}\textcolor{red}{G}\textcolor{red}{F}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{P\ }\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{P}\textcolor{red}{E}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{G}\textcolor{green}{G}\textcolor{red}{A}\textcolor{red}{R\ }\textcolor{green}{H}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{W}\textcolor{green}{D}\textcolor{red}{V}\textcolor{red}{N}\textcolor{red}{A}\textcolor{green}{N}\textcolor{red}{E\ }\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{D}\textcolor{red}{E}\textcolor{red}{E}\textcolor{red}{T}\textcolor{green}{F}\textcolor{red}{H}\textcolor{green}{N}\textcolor{black}{M\ }\textcolor{red}{L}\textcolor{red}{N}\textcolor{green}{P}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{T}\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{red}{D}\textcolor{red}{Q}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{F}\textcolor{red}{E}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{red}{N}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{W}\textcolor{black}{C}\textcolor{red}{F}\textcolor{red}{H}\textcolor{red}{G\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\\
\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R\ }\textcolor{green}{F}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{T}\textcolor{red}{D}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{S}\textcolor{red}{P}\textcolor{red}{V}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{P\ }\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{P}\textcolor{red}{F}\textcolor{red}{G}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{G}\textcolor{red}{L}\textcolor{red}{S\ }\textcolor{green}{H}\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{A}\textcolor{green}{D}\textcolor{red}{E}\textcolor{red}{D}\textcolor{red}{L}\textcolor{green}{N}\textcolor{red}{P\ }\textcolor{red}{V}\textcolor{red}{T}\textcolor{red}{I}\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{N}\textcolor{green}{F}\textcolor{red}{A}\textcolor{green}{N}\textcolor{black}{M\ }\textcolor{red}{S}\textcolor{red}{D}\textcolor{green}{P}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{L}\textcolor{red}{E}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{red}{E}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{F}\textcolor{red}{H}\textcolor{green}{H}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{red}{I}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{W}\textcolor{black}{C}\textcolor{red}{I}\textcolor{red}{G}\textcolor{red}{N\ }\\
\\
\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{P}\textcolor{black}{K}\textcolor{red}{T}\textcolor{black}{M}\textcolor{red}{T}\textcolor{red}{P}\textcolor{red}{L}\textcolor{green}{D\ }\textcolor{red}{E}\textcolor{red}{V}\textcolor{green}{V}\textcolor{black}{K}\textcolor{red}{G}\textcolor{red}{F}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{T}\textcolor{red}{P\ }\textcolor{green}{E}\textcolor{red}{A}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{T}\textcolor{green}{G}\textcolor{red}{W}\textcolor{red}{S}\textcolor{red}{R}\textcolor{red}{V\ }\textcolor{red}{D}\textcolor{black}{M}\textcolor{red}{D}\textcolor{red}{D}\textcolor{red}{W}\textcolor{red}{T}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{L}\textcolor{black}{Y\ }\textcolor{red}{I}\textcolor{black}{K}\textcolor{red}{G}\textcolor{red}{A}\textcolor{black}{M}\textcolor{red}{P}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{E}\textcolor{red}{F\ }\textcolor{red}{Q}\textcolor{red}{H}\textcolor{black}{Y}\textcolor{red}{T}\textcolor{red}{L}\textcolor{green}{R}\textcolor{red}{H}\textcolor{red}{T}\\
\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{G}\textcolor{black}{K}\textcolor{red}{N}\textcolor{black}{M}\textcolor{red}{P}\textcolor{red}{G}\textcolor{red}{N}\textcolor{green}{D\ }\textcolor{red}{D}\textcolor{red}{L}\textcolor{green}{V}\textcolor{black}{K}\textcolor{red}{P}\textcolor{red}{V}\textcolor{black}{K}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{red}{A\ }\textcolor{green}{E}\textcolor{red}{N}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{D}\textcolor{green}{G}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{A}\textcolor{red}{L\ }\textcolor{red}{I}\textcolor{black}{M}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{G}\textcolor{red}{R}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{L}\textcolor{black}{Y\ }\textcolor{red}{E}\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{D}\textcolor{black}{M}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{D}\textcolor{red}{H}\textcolor{red}{I\ }\textcolor{red}{E}\textcolor{red}{S}\textcolor{black}{Y}\textcolor{red}{G}\textcolor{red}{I}\textcolor{green}{R}\textcolor{red}{S}\textcolor{red}{L}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7B5SU74.tex <==


ID = A0A7B5SU74



Description = Phage tail protein (Fragment) n=54 Tax=Escherichia coli TaxID=562 RepID=A0A7B5SU74\_ECOLX

Length = 99 (aa)

Predicted matches = 70 / 88 (79.55\%)

TM-score = 0.6245

Superposition in the TM-score: Length(d<5.0)= 64

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7B5SU74.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{K}\textcolor{green}{G}\textcolor{red}{A}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{red}{I}\textcolor{red}{N}\textcolor{red}{S}\textcolor{green}{T\ }\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{Q}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{T\ }\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{W}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{red}{A\ }\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{I}\textcolor{red}{V\ }\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{S}\textcolor{red}{E}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{red}{T}\textcolor{red}{Q}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{K\ }\textcolor{black}{Y}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{red}{P}\textcolor{red}{D}\textcolor{red}{D}\textcolor{red}{I}\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{black}{K}\textcolor{green}{G}\textcolor{red}{I}\textcolor{red}{V}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{S}\textcolor{red}{D}\textcolor{green}{T\ }\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{T\ }\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{W}\textcolor{red}{N}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{red}{P\ }\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{I}\textcolor{red}{T\ }\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{S}\textcolor{red}{T}\textcolor{green}{S\ }\textcolor{green}{E}\textcolor{red}{V}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{K\ }\textcolor{black}{Y}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{red}{A}\textcolor{red}{T}\textcolor{red}{T}\textcolor{red}{T}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7D7HQC6.tex <==


ID = A0A7D7HQC6



Description = Glycine betaine ABC transporter permease YehY n=1 Tax=Escherichia coli TaxID=562 RepID=A0A7D7HQC6\_ECOLX

Length = 385 (aa)

Predicted matches = 257 / 359 (71.59\%)

TM-score = 0.8908

Superposition in the TM-score: Length(d<5.0)= 353

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7D7HQC6.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{I}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{green}{R}\textcolor{red}{P}\textcolor{green}{N}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{A\ }\textcolor{red}{I}\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{W}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{I}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{T\ }\textcolor{red}{I}\textcolor{black}{M}\textcolor{red}{V}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{V}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{S\ }\textcolor{green}{N}\textcolor{red}{D}\textcolor{red}{S}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{G}\textcolor{red}{I}\textcolor{red}{L}\textcolor{red}{G}\textcolor{red}{D\ }\textcolor{green}{L}\textcolor{green}{W}\textcolor{red}{T}\textcolor{red}{P}\textcolor{red}{G}\textcolor{red}{V}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{red}{S}\textcolor{red}{L\ }\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{S}\textcolor{red}{D}\textcolor{red}{T}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{S\ }\textcolor{red}{A}\textcolor{red}{L}\textcolor{black}{C}\textcolor{green}{F}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{A}\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{A\ }\textcolor{green}{S}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{F\ }\textcolor{red}{V}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{W}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{red}{R}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{N}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{red}{L}\textcolor{green}{G\ }\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{S\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{A}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{green}{R}\textcolor{red}{I}\textcolor{green}{N}\textcolor{red}{P}\textcolor{red}{V}\textcolor{red}{L\ }\textcolor{red}{A}\textcolor{red}{F}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{A\ }\textcolor{red}{A}\textcolor{black}{M}\textcolor{red}{L}\textcolor{red}{P}\textcolor{red}{F}\textcolor{red}{I}\textcolor{red}{S}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{P\ }\textcolor{green}{N}\textcolor{red}{R}\textcolor{red}{L}\textcolor{green}{V}\textcolor{red}{S}\textcolor{green}{G}\textcolor{red}{E}\textcolor{red}{G}\textcolor{red}{R}\textcolor{red}{H\ }\textcolor{green}{L}\textcolor{green}{W}\textcolor{red}{Q}\textcolor{red}{L}\textcolor{red}{W}\textcolor{red}{P}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{red}{L}\textcolor{red}{W\ }\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{G}\textcolor{red}{V}\textcolor{red}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{W}\textcolor{red}{L\ }\textcolor{red}{T}\textcolor{red}{A}\textcolor{black}{C}\textcolor{green}{F}\textcolor{red}{V}\textcolor{red}{P}\textcolor{red}{G}\textcolor{black}{K}\textcolor{black}{K}\textcolor{red}{G\ }\textcolor{green}{S}\textcolor{green}{I}\textcolor{red}{F}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{F\ }\textcolor{red}{I}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{W}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{T}\textcolor{red}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{red}{N}\textcolor{green}{G\ }\textcolor{green}{S}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{R}\textcolor{red}{T}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{S\ }\\
\\
\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{red}{S}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{H}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{W\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{Q\ }\textcolor{red}{D}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{L}\textcolor{red}{D}\textcolor{red}{I\ }\textcolor{green}{W}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{Q\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{I\ }\textcolor{red}{T}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{H}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{W\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{Q\ }\textcolor{red}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{V\ }\textcolor{green}{W}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{red}{S}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{Q\ }\\
\\
\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{G}\textcolor{green}{L}\textcolor{red}{P}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{A\ }\textcolor{green}{A}\textcolor{red}{Q}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{A\ }\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{red}{S}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{red}{P}\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{red}{H}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{W}\textcolor{green}{L\ }\textcolor{red}{L}\textcolor{red}{P}\textcolor{red}{S}\textcolor{black}{M}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{S}\textcolor{red}{L}\textcolor{green}{Q\ }\textcolor{red}{E}\textcolor{green}{P}\textcolor{red}{P}\textcolor{red}{A}\textcolor{red}{W}\textcolor{green}{L}\textcolor{green}{E}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{S}\textcolor{red}{D}\textcolor{red}{V}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{F\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{V}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{W}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{P}\textcolor{green}{S}\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{A}\textcolor{red}{P}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{T\ }\textcolor{green}{A}\textcolor{red}{F}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{V\ }\textcolor{green}{A}\textcolor{red}{G}\textcolor{red}{T}\textcolor{green}{G}\textcolor{black}{M}\textcolor{red}{T}\textcolor{red}{P}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{P}\textcolor{green}{L\ }\textcolor{red}{V}\textcolor{red}{R}\textcolor{red}{G}\textcolor{black}{M}\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{N}\textcolor{green}{Q\ }\textcolor{red}{I}\textcolor{green}{P}\textcolor{red}{R}\textcolor{red}{D}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{S}\textcolor{red}{G}\textcolor{red}{A}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{F\ }\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{black}{M\ }\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{T}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A\ }\\
\\
\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{red}{G}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{H}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{red}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{I}\textcolor{red}{P}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{red}{I}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{D}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{S}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{red}{D}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{V}\textcolor{green}{I}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{green}{F}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{D}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7H9LRP9.tex <==


ID = A0A7H9LRP9



Description = DUF1482 family protein n=3 Tax=Escherichia coli TaxID=562 RepID=A0A7H9LRP9\_ECOLX

Length = 67 (aa)

Predicted matches = 50 / 56 (89.29\%)

TM-score = 0.7125

Superposition in the TM-score: Length(d<5.0)= 51

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7H9LRP9.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{T}\textcolor{red}{E}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{red}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{H}\textcolor{red}{V}\textcolor{green}{S}\textcolor{black}{M}\textcolor{black}{K\ }\textcolor{green}{E}\textcolor{black}{C}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{red}{V}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{N}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{K\ }\textcolor{red}{P}\textcolor{green}{I}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{P}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{T}\textcolor{red}{G}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{H}\textcolor{red}{D}\textcolor{green}{S}\textcolor{black}{M}\textcolor{black}{K\ }\textcolor{green}{E}\textcolor{black}{C}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{red}{I}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{N}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{K\ }\textcolor{red}{V}\textcolor{green}{I}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{P}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7H9LWZ7.tex <==


ID = A0A7H9LWZ7



Description = Protein deglycase HchA n=1 Tax=Escherichia coli TaxID=562 RepID=A0A7H9LWZ7\_ECOLX

Length = 283 (aa)

Predicted matches = 188 / 242 (77.69\%)

TM-score = 0.9243

Superposition in the TM-score: Length(d<5.0)= 266

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7H9LWZ7.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{T}\textcolor{red}{T}\textcolor{green}{Q}\textcolor{red}{I}\textcolor{red}{G}\textcolor{black}{K}\textcolor{green}{N}\textcolor{red}{I}\textcolor{red}{A\ }\textcolor{red}{V}\textcolor{green}{D}\textcolor{black}{M}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{T}\textcolor{red}{E}\textcolor{red}{L}\textcolor{red}{I}\textcolor{green}{F\ }\textcolor{red}{S}\textcolor{red}{F}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{red}{D}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{V}\textcolor{green}{S}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{black}{Y}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{red}{R}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{H}\textcolor{black}{K\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{I}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{P\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{Q}\textcolor{red}{Q}\textcolor{red}{S}\textcolor{black}{K}\textcolor{green}{N}\textcolor{red}{P}\textcolor{red}{Q\ }\textcolor{red}{I}\textcolor{green}{D}\textcolor{black}{M}\textcolor{red}{A}\textcolor{red}{E}\textcolor{red}{D}\textcolor{red}{N}\textcolor{red}{A}\textcolor{red}{F}\textcolor{green}{F\ }\textcolor{red}{P}\textcolor{red}{S}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{red}{S}\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{I}\textcolor{green}{S}\textcolor{red}{D}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{black}{Y}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{red}{S}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{Q}\textcolor{black}{K\ }\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{R}\textcolor{black}{Y\ }\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{T}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{P\ }\\
\\
\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{red}{D}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{F\ }\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{G}\textcolor{red}{D}\textcolor{red}{I}\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{A\ }\textcolor{red}{E}\textcolor{red}{T}\textcolor{green}{E}\textcolor{red}{E}\textcolor{black}{K}\textcolor{red}{G}\textcolor{red}{S}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{red}{Q}\textcolor{red}{G}\textcolor{red}{I}\textcolor{red}{P}\textcolor{red}{T}\textcolor{green}{E}\textcolor{red}{A}\textcolor{red}{N}\textcolor{green}{R}\textcolor{red}{L\ }\textcolor{red}{A}\textcolor{green}{I}\textcolor{red}{A}\textcolor{red}{D}\textcolor{black}{C}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{W}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{P\ }\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{I\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{I}\textcolor{green}{F\ }\textcolor{green}{V}\textcolor{red}{P}\textcolor{green}{G}\textcolor{red}{G}\textcolor{red}{H}\textcolor{red}{G}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{I}\textcolor{red}{G\ }\textcolor{red}{L}\textcolor{red}{P}\textcolor{green}{E}\textcolor{red}{S}\textcolor{black}{K}\textcolor{red}{D}\textcolor{red}{V}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{red}{Q}\textcolor{red}{W}\textcolor{red}{A}\textcolor{red}{I}\textcolor{green}{E}\textcolor{red}{N}\textcolor{red}{D}\textcolor{green}{R}\textcolor{red}{F\ }\textcolor{red}{V}\textcolor{green}{I}\textcolor{red}{S}\textcolor{red}{L}\textcolor{black}{C}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{P\ }\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{I\ }\\
\\
\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{L}\textcolor{red}{N}\textcolor{green}{W}\textcolor{black}{Y\ }\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{M\ }\textcolor{green}{N}\textcolor{green}{I}\textcolor{red}{I}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{green}{V}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{black}{Y}\textcolor{red}{A}\textcolor{red}{S}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{W}\textcolor{black}{Y\ }\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{M\ }\textcolor{green}{N}\textcolor{green}{I}\textcolor{red}{V}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{green}{V}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{black}{Y}\textcolor{red}{V}\textcolor{red}{G}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A7H9QJ10.tex <==


ID = A0A7H9QJ10



Description = Putative aminohydrolase SsnA n=1 Tax=Escherichia coli TaxID=562 RepID=A0A7H9QJ10\_ECOLX

Length = 442 (aa)

Predicted matches = 307 / 386 (79.53\%)

TM-score = 0.9813

Superposition in the TM-score: Length(d<5.0)= 437

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A7H9QJ10.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{A}\textcolor{green}{V}\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{P}\textcolor{red}{T}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{red}{R\ }\textcolor{red}{N}\textcolor{red}{A}\textcolor{red}{Q}\textcolor{red}{V}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{V\ }\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{A}\textcolor{red}{A}\textcolor{red}{G}\textcolor{green}{A}\textcolor{red}{V}\textcolor{red}{G}\textcolor{red}{E}\textcolor{green}{R\ }\textcolor{red}{H}\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{F}\textcolor{red}{D}\textcolor{black}{K}\textcolor{red}{N}\textcolor{black}{M}\textcolor{red}{I\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{red}{H}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{P}\textcolor{red}{I}\textcolor{red}{L}\textcolor{green}{V}\textcolor{black}{C\ }\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{L\ }\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{P}\textcolor{black}{C\ }\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{L\ }\textcolor{red}{S}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{black}{C\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{N}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{red}{Q}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{P}\textcolor{red}{A}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{red}{G\ }\textcolor{red}{V}\textcolor{red}{D}\textcolor{red}{I}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{E}\textcolor{red}{N}\textcolor{red}{D}\textcolor{red}{V}\textcolor{red}{I\ }\textcolor{red}{V}\textcolor{green}{A}\textcolor{red}{I}\textcolor{red}{G}\textcolor{red}{D}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{Q}\textcolor{green}{R\ }\textcolor{red}{F}\textcolor{red}{P}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{S}\textcolor{red}{F}\textcolor{black}{K}\textcolor{red}{E}\textcolor{black}{M}\textcolor{red}{H\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{red}{I}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{P}\textcolor{red}{G}\textcolor{red}{I}\textcolor{green}{V}\textcolor{black}{C\ }\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{H}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{red}{S\ }\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{P}\textcolor{black}{C\ }\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{L\ }\textcolor{red}{W}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{black}{C\ }\\
\\
\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{A\ }\textcolor{black}{Y}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{red}{D}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{N\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{red}{R}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{I}\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{I\ }\textcolor{green}{D}\textcolor{red}{E}\textcolor{red}{E}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{E}\textcolor{green}{P\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{H\ }\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{T\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{H}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{P}\textcolor{red}{D\ }\textcolor{black}{Y}\textcolor{green}{I}\textcolor{red}{G}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{V}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{N\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{red}{I}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{V\ }\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{I}\textcolor{red}{R}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{I\ }\textcolor{green}{D}\textcolor{red}{N}\textcolor{red}{A}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{P\ }\textcolor{black}{Y}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{H\ }\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{T\ }\\
\\
\textcolor{red}{D}\textcolor{green}{R}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{I}\textcolor{red}{A}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E\ }\textcolor{green}{D}\textcolor{red}{A}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{red}{G}\textcolor{red}{G}\textcolor{red}{R}\textcolor{red}{E}\textcolor{green}{H}\textcolor{red}{S\ }\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{T}\textcolor{red}{N}\textcolor{red}{A}\textcolor{red}{N}\textcolor{green}{R}\textcolor{red}{I\ }\textcolor{red}{D}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{red}{D}\textcolor{red}{D}\textcolor{green}{D}\textcolor{red}{E}\textcolor{black}{K}\textcolor{green}{T\ }\textcolor{red}{Q}\textcolor{green}{V}\textcolor{red}{E}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{red}{P}\textcolor{red}{R}\textcolor{black}{K\ }\textcolor{red}{D}\textcolor{green}{D}\textcolor{red}{E}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{F}\textcolor{red}{H}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{S}\textcolor{red}{S\ }\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{N}\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{red}{I}\textcolor{green}{H}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{H}\textcolor{red}{V\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{red}{G}\textcolor{green}{R}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{H}\textcolor{green}{I}\textcolor{red}{H}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E\ }\textcolor{green}{D}\textcolor{red}{L}\textcolor{black}{Y}\textcolor{red}{D}\textcolor{red}{V}\textcolor{red}{S}\textcolor{red}{H}\textcolor{red}{S}\textcolor{green}{H}\textcolor{red}{H\ }\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{A}\textcolor{green}{R}\textcolor{red}{L\ }\textcolor{red}{A}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{red}{L}\textcolor{red}{I}\textcolor{green}{D}\textcolor{red}{S}\textcolor{black}{K}\textcolor{green}{T\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{H}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{red}{S}\textcolor{black}{K\ }\textcolor{red}{E}\textcolor{green}{D}\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{F}\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{S}\textcolor{red}{N\ }\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{N}\textcolor{red}{H}\textcolor{green}{V}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{red}{N}\textcolor{green}{H}\textcolor{green}{H\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{H}\textcolor{red}{R\ }\\
\\
\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{S\ }\textcolor{green}{F}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{G}\textcolor{red}{D}\textcolor{green}{E\ }\textcolor{red}{Q}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{F\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{red}{S}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{H\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{D}\textcolor{black}{C\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{D}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{S\ }\textcolor{green}{F}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{E\ }\textcolor{red}{L}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{F\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{red}{H}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{H\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{H}\textcolor{green}{S}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{V\ }\textcolor{black}{Y}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{F}\textcolor{green}{D}\textcolor{black}{C\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{I}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{K}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{W}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{D}\textcolor{green}{A\ }\\
\\
\textcolor{green}{L}\textcolor{green}{A}\\
\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{L}\textcolor{green}{A}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A811CCH1.tex <==


ID = A0A811CCH1



Description = Nitrogen fixation protein rnfC n=1 Tax=Escherichia coli TaxID=562 RepID=A0A811CCH1\_ECOLX

Length = 447 (aa)

Predicted matches = 347 / 404 (85.89\%)

TM-score = 0.9787

Superposition in the TM-score: Length(d<5.0)= 444

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A811CCH1.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{red}{I}\textcolor{black}{K}\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{I}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{D\ }\textcolor{red}{T}\textcolor{green}{T}\textcolor{red}{F}\textcolor{red}{I}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{red}{Q}\textcolor{green}{V}\textcolor{red}{N}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{P}\textcolor{green}{T}\textcolor{red}{Q}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{C\ }\textcolor{green}{E}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{H\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{red}{V}\textcolor{black}{K}\textcolor{red}{L}\textcolor{red}{T}\textcolor{red}{S}\textcolor{black}{C}\textcolor{green}{D}\textcolor{green}{D\ }\textcolor{red}{Q}\textcolor{green}{T}\textcolor{red}{I}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{red}{G}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{P}\textcolor{green}{T}\textcolor{red}{H}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{C\ }\textcolor{green}{E}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R\ }\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{red}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{H\ }\\
\\
\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{V\ }\textcolor{red}{N}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{E\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{red}{T}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{P}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{T}\textcolor{green}{S\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{I}\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{V\ }\textcolor{red}{S}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{Q\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{E\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{L\ }\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{P}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{T}\textcolor{green}{S\ }\\
\\
\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{S\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{C\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{T}\textcolor{green}{D}\textcolor{red}{Q}\textcolor{black}{C\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{N}\textcolor{black}{Y\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{V\ }\textcolor{black}{C}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{H}\textcolor{green}{S\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{Q}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{C\ }\textcolor{green}{E}\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{T}\textcolor{green}{D}\textcolor{red}{L}\textcolor{black}{C\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{N}\textcolor{black}{Y\ }\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{T}\textcolor{black}{C}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{N}\textcolor{green}{V\ }\textcolor{black}{C}\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K\ }\\
\\
\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{Y\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{P}\textcolor{black}{M\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{K}\textcolor{red}{R\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{W\ }\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{red}{A}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{V}\textcolor{red}{A}\textcolor{red}{V}\textcolor{green}{L\ }\textcolor{red}{L}\textcolor{red}{E}\textcolor{red}{G}\textcolor{red}{F}\textcolor{red}{V}\textcolor{red}{I}\textcolor{red}{V}\textcolor{red}{T}\textcolor{red}{P}\textcolor{red}{L\ }\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{L}\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{Q}\textcolor{red}{V}\textcolor{red}{G}\textcolor{red}{R}\textcolor{red}{F\ }\textcolor{red}{D}\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{G}\textcolor{red}{T}\textcolor{red}{Q}\textcolor{green}{P}\textcolor{red}{N}\textcolor{red}{E\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{P}\textcolor{red}{F}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I\ }\textcolor{red}{E}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{N\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{Y\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{P}\textcolor{black}{M\ }\textcolor{green}{A}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{I}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{K}\textcolor{red}{Q\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{W\ }\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{Q}\textcolor{green}{V\ }\textcolor{green}{P}\textcolor{green}{Q}\textcolor{red}{P}\textcolor{green}{E}\textcolor{black}{K}\textcolor{red}{V}\textcolor{red}{T}\textcolor{red}{L}\textcolor{red}{L}\textcolor{green}{L\ }\textcolor{red}{R}\textcolor{red}{Q}\textcolor{red}{H}\textcolor{red}{I}\textcolor{red}{G}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{A\ }\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{Q}\textcolor{black}{K}\textcolor{red}{G}\textcolor{red}{D}\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{V}\textcolor{red}{H\ }\textcolor{red}{G}\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{G}\textcolor{red}{Q}\textcolor{red}{I}\textcolor{green}{P}\textcolor{red}{H}\textcolor{red}{G\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{P}\textcolor{red}{I}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I\ }\textcolor{red}{D}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{N\ }\\
\\
\textcolor{red}{R}\textcolor{red}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{G}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{red}{A}\textcolor{red}{I}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{G}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A826NIQ8.tex <==


ID = A0A826NIQ8



Description = Host specificity protein J (Fragment) n=1 Tax=Escherichia coli TaxID=562 RepID=A0A826NIQ8\_ECOLX

Length = 338 (aa)

Predicted matches = 236 / 302 (78.15\%)

TM-score = 0.8801

Superposition in the TM-score: Length(d<5.0)= 321

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A826NIQ8.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{red}{V}\textcolor{red}{T}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{P}\textcolor{green}{I}\textcolor{red}{E}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{V}\textcolor{red}{G\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{R}\textcolor{red}{E}\textcolor{red}{D\ }\textcolor{red}{G}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{G}\textcolor{red}{L}\textcolor{red}{I}\textcolor{green}{N\ }\textcolor{green}{I}\textcolor{red}{F}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{P}\textcolor{green}{F}\textcolor{green}{R}\textcolor{red}{Q\ }\textcolor{green}{G}\textcolor{red}{G}\textcolor{red}{E}\textcolor{red}{T}\textcolor{red}{T}\textcolor{red}{P}\textcolor{green}{P}\textcolor{green}{P}\textcolor{red}{T}\textcolor{green}{G\ }\textcolor{green}{F}\textcolor{red}{S}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{I}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{I}\textcolor{red}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{D\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{T\ }\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{S\ }\textcolor{green}{T}\textcolor{red}{Q}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{G}\textcolor{green}{P}\textcolor{green}{I}\textcolor{red}{Q}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{V}\textcolor{red}{D\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{N}\textcolor{red}{G}\textcolor{red}{T\ }\textcolor{red}{P}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{S}\textcolor{green}{E}\textcolor{green}{G}\textcolor{red}{N}\textcolor{red}{T}\textcolor{green}{N\ }\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{G}\textcolor{red}{V}\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{F}\textcolor{green}{R}\textcolor{red}{A\ }\textcolor{green}{G}\textcolor{red}{E}\textcolor{red}{Q}\textcolor{red}{E}\textcolor{red}{Q}\textcolor{red}{T}\textcolor{green}{P}\textcolor{green}{P}\textcolor{red}{E}\textcolor{green}{G\ }\textcolor{green}{F}\textcolor{red}{E}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{E}\textcolor{red}{T}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{V}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{I\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{I}\textcolor{red}{T}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{D\ }\\
\\
\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{F}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{Q\ }\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{red}{F}\textcolor{black}{Y}\textcolor{red}{G}\textcolor{green}{A}\textcolor{green}{S}\textcolor{red}{D}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{F}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{R\ }\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{T}\textcolor{red}{R\ }\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{Q\ }\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{red}{L\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{T}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{S}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{R\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{Q\ }\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{red}{Q}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{S}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{D\ }\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{F}\textcolor{red}{S}\textcolor{green}{I}\textcolor{green}{R\ }\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{T}\textcolor{red}{T\ }\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{S\ }\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{Q\ }\textcolor{black}{C}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{G}\textcolor{red}{V\ }\\
\\
\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{Q}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{V}\textcolor{red}{R}\textcolor{green}{S}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{N\ }\textcolor{green}{P}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{W\ }\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{N\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{W}\textcolor{black}{C}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R\ }\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{W}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{D}\textcolor{red}{N\ }\textcolor{red}{T}\textcolor{red}{R}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{G}\textcolor{red}{N}\textcolor{green}{G}\textcolor{red}{G}\textcolor{red}{N\ }\textcolor{red}{R}\textcolor{red}{S}\textcolor{red}{F}\textcolor{red}{S}\textcolor{black}{C}\textcolor{red}{L}\textcolor{green}{A}\textcolor{red}{R}\textcolor{red}{R}\textcolor{red}{E\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{red}{F}\textcolor{green}{R}\textcolor{green}{G\ }\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{green}{V}\textcolor{red}{P}\textcolor{green}{S}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{N\ }\textcolor{green}{P}\textcolor{green}{Q}\textcolor{red}{T}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{W\ }\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{F}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{D\ }\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{W}\textcolor{black}{C}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R\ }\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{W}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{red}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{D}\textcolor{red}{Q\ }\textcolor{red}{S}\textcolor{red}{V}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{S}\textcolor{red}{G}\textcolor{green}{G}\textcolor{red}{T}\textcolor{red}{E\ }\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{I}\textcolor{red}{T}\textcolor{black}{C}\textcolor{red}{N}\textcolor{green}{A}\textcolor{red}{W}\textcolor{red}{L}\textcolor{red}{T\ }\\
\\
\textcolor{red}{W}\textcolor{red}{F}\textcolor{red}{E}\textcolor{black}{K}\textcolor{red}{I}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{T}\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{red}{R}\textcolor{red}{Q}\textcolor{red}{R}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{W}\textcolor{red}{D}\textcolor{red}{V}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A827JW37.tex <==


ID = A0A827JW37



Description = M28 family peptidase n=2 Tax=Escherichia TaxID=561 RepID=A0A827JW37\_ECOLX

Length = 323 (aa)

Predicted matches = 223 / 285 (78.25\%)

TM-score = 0.851

Superposition in the TM-score: Length(d<5.0)= 275

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A827JW37.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{N}\textcolor{green}{F}\textcolor{red}{A}\textcolor{green}{F}\textcolor{red}{I}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{I\ }\textcolor{red}{A}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{green}{T}\textcolor{green}{Q\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{I\ }\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{I\ }\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{I}\textcolor{red}{F\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{I}\textcolor{red}{T}\textcolor{green}{F}\textcolor{red}{P}\textcolor{green}{F}\textcolor{red}{F}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{I}\textcolor{red}{V\ }\textcolor{red}{F}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{P}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{red}{F}\textcolor{green}{T}\textcolor{green}{Q\ }\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{I\ }\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{I\ }\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{R\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{Q}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{Y\ }\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{G}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{I}\textcolor{red}{I\ }\\
\\
\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{S}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{red}{T}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{H}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{red}{V}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{H\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{Y\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{red}{T}\textcolor{red}{P}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{red}{N}\textcolor{black}{Y}\textcolor{green}{P\ }\textcolor{black}{Y}\textcolor{red}{P}\textcolor{red}{A}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{D\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{S}\textcolor{red}{A}\textcolor{red}{T}\textcolor{green}{S}\textcolor{black}{Y\ }\textcolor{green}{E}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{red}{I}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{G\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{green}{Q\ }\textcolor{green}{Q}\textcolor{red}{A}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{F\ }\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{H\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{L\ }\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{Y\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{red}{A}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{red}{D}\textcolor{black}{Y}\textcolor{green}{P\ }\textcolor{black}{Y}\textcolor{red}{S}\textcolor{red}{V}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{D\ }\\
\\
\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{black}{M}\textcolor{red}{T}\textcolor{green}{D}\textcolor{green}{I}\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{red}{L\ }\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{E}\textcolor{green}{L}\textcolor{red}{P}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{L\ }\textcolor{red}{F}\textcolor{red}{P}\textcolor{black}{Y}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{N}\textcolor{red}{G}\textcolor{red}{I}\textcolor{green}{F\ }\textcolor{red}{Q}\textcolor{red}{N}\textcolor{green}{G}\textcolor{red}{W}\textcolor{red}{A}\textcolor{green}{F}\textcolor{red}{A}\textcolor{red}{N}\textcolor{green}{H}\textcolor{red}{V\ }\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{red}{H}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N\ }\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{red}{L}\textcolor{red}{P}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A\ }\textcolor{green}{D}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{A}\textcolor{red}{E\ }\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{W}\textcolor{red}{S}\textcolor{red}{L}\textcolor{red}{F}\textcolor{green}{S}\textcolor{red}{G}\textcolor{red}{E}\textcolor{red}{E\ }\textcolor{red}{R}\textcolor{red}{N}\textcolor{black}{K}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{black}{M}\textcolor{red}{Q}\textcolor{green}{D}\textcolor{green}{I}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{red}{V\ }\textcolor{black}{K}\textcolor{red}{S}\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{A}\textcolor{red}{T}\textcolor{red}{E}\textcolor{green}{L\ }\textcolor{red}{P}\textcolor{red}{V}\textcolor{black}{Y}\textcolor{red}{S}\textcolor{red}{I}\textcolor{red}{N}\textcolor{red}{A}\textcolor{red}{P}\textcolor{red}{G}\textcolor{green}{F\ }\textcolor{red}{I}\textcolor{red}{P}\textcolor{green}{G}\textcolor{red}{I}\textcolor{red}{D}\textcolor{green}{F}\textcolor{red}{S}\textcolor{red}{D}\textcolor{green}{H}\textcolor{red}{L\ }\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{red}{Q}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{N\ }\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{H}\textcolor{red}{Q}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{A\ }\textcolor{green}{D}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{A}\textcolor{red}{Q\ }\textcolor{red}{V}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{G}\textcolor{red}{V}\textcolor{red}{I}\textcolor{green}{S}\textcolor{red}{L}\textcolor{red}{L}\textcolor{red}{H\ }\textcolor{red}{N}\textcolor{red}{S}\textcolor{black}{K}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A827K0J7.tex <==


ID = A0A827K0J7



Description = TIGR01777 family protein n=1 Tax=Escherichia coli TaxID=562 RepID=A0A827K0J7\_ECOLX

Length = 297 (aa)

Predicted matches = 228 / 274 (83.21\%)

TM-score = 0.9629

Superposition in the TM-score: Length(d<5.0)= 286

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A827K0J7.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{red}{I}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{N}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{P}\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{red}{S}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{red}{A}\textcolor{green}{V}\textcolor{red}{I}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{P\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{black}{K}\textcolor{red}{E}\textcolor{red}{R}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{N\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{D}\textcolor{red}{T}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{R}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{red}{V}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{V\ }\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{T}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{P}\textcolor{red}{Q}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{G\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{red}{R}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{V\ }\textcolor{green}{D}\textcolor{red}{V}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{P\ }\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{E}\textcolor{green}{Q\ }\textcolor{black}{K}\textcolor{red}{D}\textcolor{red}{L}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{N\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{D}\textcolor{red}{S}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I\ }\\
\\
\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{L\ }\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{G}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P\ }\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{W}\textcolor{green}{I}\textcolor{green}{H\ }\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{W\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{N}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{P}\textcolor{red}{G\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{D\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{E\ }\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{N}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{H}\textcolor{black}{K}\textcolor{green}{L\ }\textcolor{black}{C}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{W}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{I}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{S}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{red}{S}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{P\ }\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{G\ }\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{red}{P}\textcolor{green}{W}\textcolor{green}{I}\textcolor{green}{H\ }\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{W\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{N}\textcolor{red}{D}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{P}\textcolor{red}{F\ }\\
\\
\textcolor{green}{N}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{red}{R}\textcolor{red}{R}\textcolor{green}{N\ }\textcolor{red}{V}\textcolor{red}{P}\textcolor{red}{L}\textcolor{red}{D}\textcolor{red}{Q}\textcolor{red}{G}\textcolor{red}{I}\textcolor{red}{T}\textcolor{red}{S}\textcolor{red}{L\ }\textcolor{red}{V}\textcolor{green}{H}\textcolor{red}{I}\textcolor{red}{S}\textcolor{red}{I}\textcolor{red}{V}\textcolor{black}{M}\textcolor{red}{T}\textcolor{red}{R}\textcolor{red}{H\ }\textcolor{red}{G}\textcolor{red}{N}\textcolor{green}{A}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{S}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{G}\textcolor{red}{S\ }\textcolor{green}{S}\textcolor{red}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{D}\textcolor{red}{P}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{F}\textcolor{red}{S}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{E\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{R}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{N}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{red}{V}\textcolor{red}{H}\textcolor{green}{N\ }\textcolor{red}{E}\textcolor{red}{Q}\textcolor{red}{F}\textcolor{red}{A}\textcolor{red}{H}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{G}\textcolor{red}{H}\textcolor{red}{A\ }\textcolor{red}{L}\textcolor{green}{H}\textcolor{red}{R}\textcolor{red}{P}\textcolor{red}{A}\textcolor{red}{I}\textcolor{black}{M}\textcolor{red}{R}\textcolor{red}{V}\textcolor{red}{P\ }\textcolor{red}{A}\textcolor{red}{A}\textcolor{green}{A}\textcolor{red}{I}\textcolor{red}{R}\textcolor{red}{L}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{G}\textcolor{red}{E\ }\textcolor{green}{S}\textcolor{red}{S}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{V}\textcolor{red}{L}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{R\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{F}\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{W}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{E\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{R}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A827QIW8.tex <==


ID = A0A827QIW8



Description = Phage tail protein (Fragment) n=2 Tax=Escherichia coli TaxID=562 RepID=A0A827QIW8\_ECOLX

Length = 212 (aa)

Predicted matches = 153 / 187 (81.82\%)

TM-score = 0.776

Superposition in the TM-score: Length(d<5.0)= 167

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A827QIW8.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{L}\textcolor{red}{E}\textcolor{green}{P}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{V}\textcolor{black}{Y\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{L\ }\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{W}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{W}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{W}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{I\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{P}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{N}\textcolor{green}{P}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{V\ }\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{W}\textcolor{green}{V}\textcolor{black}{Y\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{P\ }\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{M\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{S}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{N}\textcolor{black}{Y}\textcolor{green}{L\ }\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{W}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{G}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{T\ }\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{W}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{W}\textcolor{green}{F\ }\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{I\ }\\
\\
\textcolor{green}{R}\textcolor{green}{F}\textcolor{red}{P}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{W}\textcolor{red}{V}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{A\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{T}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{T\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{V}\textcolor{red}{Q}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{S\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{E}\textcolor{red}{N}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{I}\textcolor{red}{E}\textcolor{red}{E\ }\textcolor{red}{N}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{K}\textcolor{red}{D}\textcolor{green}{T}\textcolor{red}{T}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{red}{D}\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{I}\textcolor{black}{K}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{red}{T}\textcolor{red}{R}\textcolor{green}{P}\textcolor{green}{E}\textcolor{red}{N}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{T}\textcolor{red}{P}\textcolor{red}{T}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{D}\textcolor{green}{A\ }\textcolor{red}{Q}\textcolor{red}{G}\textcolor{red}{G}\textcolor{green}{T}\textcolor{red}{E}\textcolor{red}{D}\textcolor{red}{V}\textcolor{red}{D}\textcolor{red}{E}\textcolor{black}{K\ }\textcolor{red}{S}\textcolor{black}{M}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{green}{R}\textcolor{green}{F}\textcolor{red}{L}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{W}\textcolor{red}{I}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{A\ }\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{A}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{T\ }\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{V}\textcolor{red}{G}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{S\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{red}{E}\textcolor{green}{E}\textcolor{red}{R}\textcolor{red}{S}\textcolor{green}{E}\textcolor{green}{I}\textcolor{red}{T}\textcolor{red}{P\ }\textcolor{red}{A}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{K}\textcolor{red}{V}\textcolor{green}{T}\textcolor{red}{P}\textcolor{green}{T}\textcolor{green}{S\ }\textcolor{red}{G}\textcolor{green}{T}\textcolor{green}{V}\textcolor{red}{E}\textcolor{black}{K}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{V}\textcolor{green}{S}\textcolor{red}{F}\textcolor{red}{E}\textcolor{green}{P}\textcolor{green}{E}\textcolor{red}{S}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{T}\textcolor{red}{F}\textcolor{red}{R}\textcolor{red}{A}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{A\ }\textcolor{red}{D}\textcolor{red}{P}\textcolor{red}{S}\textcolor{green}{T}\textcolor{red}{G}\textcolor{red}{T}\textcolor{red}{I}\textcolor{red}{A}\textcolor{red}{V}\textcolor{black}{K\ }\textcolor{red}{D}\textcolor{black}{M}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/A0A827VWZ9.tex <==


ID = A0A827VWZ9



Description = DUF1418 family protein n=1 Tax=Escherichia coli TaxID=562 RepID=A0A827VWZ9\_ECOLX

Length = 95 (aa)

Predicted matches = 75 / 84 (89.29\%)

TM-score = 0.6211

Superposition in the TM-score: Length(d<5.0)= 79

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/A0A827VWZ9.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{I}\textcolor{green}{P}\textcolor{black}{K}\textcolor{red}{G\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{black}{M\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{S\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{red}{G}\textcolor{green}{S}\textcolor{red}{R}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{R}\textcolor{red}{E}\textcolor{green}{E}\textcolor{red}{G}\textcolor{red}{E}\textcolor{green}{I}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{F\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{N}\textcolor{red}{E}\textcolor{green}{P}\textcolor{green}{P\ }\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{D\ }\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{H}\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{black}{M}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{red}{L}\textcolor{green}{P}\textcolor{black}{K}\textcolor{red}{S\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{G}\textcolor{black}{M}\textcolor{black}{M\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{V}\textcolor{green}{S\ }\textcolor{green}{D}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{S}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{S\ }\textcolor{green}{R}\textcolor{red}{P}\textcolor{green}{E}\textcolor{red}{V}\textcolor{red}{Q}\textcolor{green}{I}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{I}\textcolor{green}{F\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{A\ }\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{R\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{N}\textcolor{red}{R}\textcolor{green}{P}\textcolor{green}{P\ }\textcolor{green}{Q}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{D\ }\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{H}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/B6VP20.tex <==


ID = B6VP20



Description = IS1294 transposase n=25 Tax=Enterobacterales TaxID=91347 RepID=B6VP20\_ECOLX

Length = 402 (aa)

Predicted matches = 282 / 332 (84.94\%)

TM-score = 0.9609

Superposition in the TM-score: Length(d<5.0)= 387

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/B6VP20.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{P\ }\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{N\ }\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{E}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{T}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{E\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{C}\textcolor{green}{D}\textcolor{black}{K\ }\textcolor{green}{P}\textcolor{red}{D}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{H}\textcolor{red}{A}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{T\ }\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{S\ }\textcolor{black}{C}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{W}\textcolor{red}{T\ }\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{N}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{Q}\textcolor{green}{D}\textcolor{black}{C\ }\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{P\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{Q}\textcolor{green}{P\ }\textcolor{green}{R}\textcolor{green}{P}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{N\ }\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{W}\textcolor{green}{T}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{D}\textcolor{green}{I}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{V\ }\textcolor{green}{T}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{T}\textcolor{green}{R}\textcolor{red}{I\ }\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{black}{C}\textcolor{green}{D}\textcolor{black}{K\ }\textcolor{green}{P}\textcolor{red}{E}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{H}\textcolor{red}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{green}{T\ }\textcolor{green}{N}\textcolor{green}{S}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{P}\textcolor{green}{S\ }\textcolor{black}{C}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{L}\textcolor{green}{W}\textcolor{red}{I\ }\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{N}\textcolor{red}{R}\textcolor{green}{L}\textcolor{red}{P}\textcolor{green}{D}\textcolor{black}{C\ }\textcolor{green}{D}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{P\ }\\
\\
\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{P}\textcolor{red}{L}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{S}\textcolor{red}{R\ }\textcolor{red}{I}\textcolor{green}{W}\textcolor{green}{L}\textcolor{red}{H}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{Q}\textcolor{black}{C}\textcolor{red}{T}\textcolor{red}{P\ }\textcolor{green}{A}\textcolor{red}{P}\textcolor{red}{V}\textcolor{green}{N}\textcolor{green}{L}\textcolor{red}{V}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{F}\textcolor{black}{C\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{L}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{V\ }\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{S}\textcolor{red}{A}\textcolor{green}{T\ }\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{K}\textcolor{red}{R}\textcolor{green}{G}\textcolor{red}{Q}\textcolor{green}{W\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{D}\textcolor{red}{G}\textcolor{black}{M\ }\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{W}\textcolor{black}{M}\textcolor{red}{L}\textcolor{red}{G}\textcolor{black}{M}\textcolor{green}{R}\textcolor{red}{G\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{V}\textcolor{red}{S}\textcolor{red}{G}\textcolor{red}{A}\textcolor{red}{L}\textcolor{red}{E\ }\textcolor{red}{E}\textcolor{black}{M}\textcolor{red}{E}\textcolor{green}{E}\textcolor{red}{F}\textcolor{red}{G}\textcolor{red}{A}\textcolor{red}{S}\textcolor{red}{N}\textcolor{green}{T\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\\
\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{L}\textcolor{red}{W}\textcolor{green}{P}\textcolor{red}{V}\textcolor{green}{F}\textcolor{green}{E}\textcolor{green}{S}\textcolor{red}{N\ }\textcolor{red}{R}\textcolor{green}{W}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{V}\textcolor{black}{C}\textcolor{red}{R}\textcolor{red}{L\ }\textcolor{green}{A}\textcolor{red}{V}\textcolor{red}{E}\textcolor{green}{N}\textcolor{green}{L}\textcolor{red}{L}\textcolor{black}{Y}\textcolor{green}{A}\textcolor{red}{A}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{I}\textcolor{green}{F}\textcolor{black}{C\ }\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{R}\textcolor{green}{R}\textcolor{green}{L}\textcolor{red}{N\ }\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{S}\textcolor{red}{V}\textcolor{green}{T\ }\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{black}{K}\textcolor{red}{H}\textcolor{green}{G}\textcolor{red}{H}\textcolor{green}{W\ }\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{D}\textcolor{red}{A}\textcolor{black}{M\ }\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{W}\textcolor{black}{M}\textcolor{red}{W}\textcolor{red}{N}\textcolor{black}{M}\textcolor{green}{R}\textcolor{red}{Q\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{L}\textcolor{black}{K}\textcolor{red}{A}\textcolor{red}{W}\textcolor{red}{S}\textcolor{red}{E}\textcolor{red}{G}\textcolor{red}{L\ }\textcolor{red}{A}\textcolor{black}{M}\textcolor{red}{P}\textcolor{green}{E}\textcolor{red}{S}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{H}\textcolor{red}{I}\textcolor{green}{T\ }\\
\\
\textcolor{red}{P}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{red}{E}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{V}\textcolor{black}{Y\ }\textcolor{black}{M}\textcolor{green}{S}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{T}\textcolor{green}{N\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{K\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{F\ }\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{R}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{T\ }\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{L\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{F}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{G\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{red}{T}\textcolor{green}{E}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{red}{R}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{V}\textcolor{black}{Y\ }\textcolor{black}{M}\textcolor{green}{S}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{G}\textcolor{red}{R}\textcolor{green}{N\ }\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{K\ }\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{N}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{F\ }\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{H}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{T\ }\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{L\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{H}\textcolor{green}{I}\textcolor{green}{P}\textcolor{green}{E\ }\textcolor{black}{K}\textcolor{green}{F}\textcolor{green}{F}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{G\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{R}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{E}\textcolor{black}{K\ }\\
\\
\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{M\ }\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{C\ }\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{S\ }\textcolor{green}{R}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{red}{T\ }\textcolor{red}{F}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{black}{M\ }\textcolor{green}{P}\textcolor{green}{A}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{G}\textcolor{black}{M\ }\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{V}\textcolor{black}{C\ }\textcolor{black}{Y}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{S\ }\textcolor{green}{R}\textcolor{red}{D}\textcolor{green}{P}\textcolor{green}{F}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{G\ }\textcolor{green}{G}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{V}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{red}{A\ }\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{N}\textcolor{green}{V}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{K}\textcolor{green}{N\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{red}{D}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{black}{M\ }\textcolor{green}{P}\textcolor{green}{A}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/B7MPY2.tex <==


ID = B7MPY2



Description = Endopeptidase (Lysis protein) from bacteriophage origin n=1 Tax=Escherichia coli O81 TaxID=585397 RepID=B7MPY2\_ECO81

Length = 155 (aa)

Predicted matches = 101 / 135 (74.81\%)

TM-score = 0.8637

Superposition in the TM-score: Length(d<5.0)= 135

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/B7MPY2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{N}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{I\ }\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{L}\textcolor{red}{V}\textcolor{red}{A}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{S\ }\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{N}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{E}\textcolor{red}{E}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{red}{R}\textcolor{red}{Q}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{D\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{red}{I}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{red}{Q}\textcolor{green}{N}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{C}\textcolor{red}{P\ }\textcolor{green}{G}\textcolor{red}{A}\textcolor{red}{E}\textcolor{green}{R}\textcolor{red}{A}\textcolor{red}{F}\textcolor{red}{S}\textcolor{red}{R}\textcolor{green}{T}\textcolor{red}{A\ }\\
\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\\
\textcolor{black}{M}\textcolor{red}{S}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{I\ }\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{G}\textcolor{red}{G}\textcolor{black}{C}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{W\ }\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{T}\textcolor{red}{D}\textcolor{green}{H}\textcolor{black}{Y}\textcolor{green}{R}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{A\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{D}\textcolor{black}{K}\textcolor{black}{K\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{E}\textcolor{red}{L}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{D}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{red}{V}\textcolor{red}{R}\textcolor{green}{Q}\textcolor{green}{R}\textcolor{green}{D\ }\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{A}\textcolor{black}{K}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{R\ }\textcolor{green}{E}\textcolor{red}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{A}\textcolor{red}{E}\textcolor{green}{N}\textcolor{green}{E\ }\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{G}\textcolor{green}{R\ }\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{A}\textcolor{green}{T}\textcolor{black}{C}\textcolor{red}{S\ }\textcolor{green}{G}\textcolor{red}{T}\textcolor{red}{V}\textcolor{green}{R}\textcolor{red}{E}\textcolor{red}{A}\textcolor{red}{T}\textcolor{red}{G}\textcolor{green}{T}\textcolor{red}{S\ }\\
\\
\textcolor{red}{N}\textcolor{black}{M}\textcolor{red}{R}\textcolor{green}{N}\textcolor{red}{G}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{N}\textcolor{red}{L}\textcolor{red}{S\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{red}{T\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{red}{D}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{R\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{L}\textcolor{red}{D}\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{red}{G}\textcolor{black}{M}\textcolor{red}{D}\textcolor{green}{N}\textcolor{red}{A}\textcolor{red}{T}\textcolor{red}{G}\textcolor{red}{P}\textcolor{red}{R}\textcolor{red}{L\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{red}{T}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{red}{I\ }\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{black}{M}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{red}{E}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{R\ }\textcolor{green}{T}\textcolor{green}{Q}\textcolor{black}{C}\textcolor{green}{L}\textcolor{red}{N}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/B7ULW9.tex <==


ID = B7ULW9



Description = Predicted kinase inhibitor n=3 Tax=Escherichia coli TaxID=562 RepID=B7ULW9\_ECO27

Length = 158 (aa)

Predicted matches = 125 / 144 (86.81\%)

TM-score = 0.9869

Superposition in the TM-score: Length(d<5.0)= 158

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/B7ULW9.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L}\textcolor{red}{R}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P\ }\textcolor{red}{A}\textcolor{green}{G}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{T}\textcolor{black}{C\ }\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{W}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{K\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{P}\textcolor{black}{K\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{D\ }\textcolor{green}{G}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{R}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{F\ }\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{N}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{green}{P}\textcolor{green}{H}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{D}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{P\ }\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{S}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{T}\textcolor{black}{C\ }\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G\ }\textcolor{green}{W}\textcolor{green}{W}\textcolor{green}{H}\textcolor{green}{W}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{P}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{F\ }\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{G\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{Q}\textcolor{green}{T}\textcolor{green}{R}\textcolor{green}{T}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{G}\textcolor{black}{K\ }\textcolor{green}{T}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{P}\textcolor{green}{P}\textcolor{black}{K\ }\\
\\
\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V\ }\textcolor{red}{V}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{V}\textcolor{red}{E\ }\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{V}\textcolor{red}{D}\textcolor{red}{I}\textcolor{red}{G}\textcolor{red}{E}\textcolor{red}{S}\textcolor{red}{I}\textcolor{red}{A\ }\textcolor{red}{L}\textcolor{red}{G}\textcolor{green}{I}\textcolor{red}{W}\textcolor{red}{G}\textcolor{red}{D}\textcolor{red}{L}\textcolor{red}{W}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{G}\textcolor{green}{E}\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{V\ }\textcolor{green}{H}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{I}\textcolor{green}{D}\textcolor{green}{V\ }\textcolor{red}{D}\textcolor{green}{E}\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{S}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{V}\textcolor{red}{G\ }\textcolor{green}{F}\textcolor{green}{N}\textcolor{green}{V}\textcolor{red}{H}\textcolor{red}{F}\textcolor{red}{H}\textcolor{red}{S}\textcolor{red}{L}\textcolor{red}{A}\textcolor{red}{S\ }\textcolor{red}{A}\textcolor{red}{S}\textcolor{green}{I}\textcolor{red}{T}\textcolor{red}{A}\textcolor{red}{I}\textcolor{red}{F}\textcolor{red}{S}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/F4T8P1.tex <==


ID = F4T8P1



Description = Toxin-antitoxin system, antitoxin component, ribbon-helix-helix fold protein n=1 Tax=Escherichia coli M605 TaxID=656417 RepID=F4T8P1\_ECOLX

Length = 94 (aa)

Predicted matches = 69 / 86 (80.23\%)

TM-score = 0.7358

Superposition in the TM-score: Length(d<5.0)= 72

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/F4T8P1.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{red}{A}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{G}\textcolor{red}{N}\textcolor{green}{V\ }\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{R}\textcolor{red}{R}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{N}\textcolor{red}{D}\textcolor{green}{Q\ }\textcolor{red}{V}\textcolor{red}{Q}\textcolor{red}{E}\textcolor{red}{D}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{V}\textcolor{red}{V}\textcolor{green}{A}\textcolor{red}{S\ }\textcolor{red}{V}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{D}\textcolor{green}{D}\textcolor{red}{H}\textcolor{green}{P}\textcolor{red}{P\ }\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{R}\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{black}{M}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{black}{K}\textcolor{green}{N}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{A\ }\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{T}\textcolor{green}{A}\textcolor{green}{H}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{L\ }\textcolor{red}{P}\textcolor{black}{M}\textcolor{green}{A}\textcolor{green}{D}\textcolor{black}{K}\textcolor{green}{V}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{A\ }\textcolor{green}{A}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{G}\textcolor{red}{W}\textcolor{green}{V\ }\textcolor{green}{I}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{W}\textcolor{green}{L}\textcolor{green}{A\ }\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{R}\textcolor{red}{L}\textcolor{green}{T}\textcolor{green}{L\ }\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{V}\textcolor{green}{T}\textcolor{red}{S}\textcolor{red}{G}\textcolor{green}{Q\ }\textcolor{red}{I}\textcolor{red}{I}\textcolor{red}{D}\textcolor{red}{H}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{V}\textcolor{red}{Q}\textcolor{green}{A}\textcolor{red}{W\ }\textcolor{red}{A}\textcolor{green}{D}\textcolor{green}{S}\textcolor{green}{L}\textcolor{red}{S}\textcolor{red}{T}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{P}\textcolor{red}{L\ }\textcolor{green}{P}\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{R}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/F4T8W4.tex <==


ID = F4T8W4



Description = Protein TrbA n=1 Tax=Escherichia coli M605 TaxID=656417 RepID=F4T8W4\_ECOLX

Length = 115 (aa)

Predicted matches = 83 / 98 (84.69\%)

TM-score = 0.6277

Superposition in the TM-score: Length(d<5.0)= 93

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/F4T8W4.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{T\ }\textcolor{red}{R}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{F}\textcolor{red}{I}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{I\ }\textcolor{red}{V}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{L}\textcolor{black}{Y\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{L}\textcolor{red}{S}\textcolor{red}{L}\textcolor{red}{P}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{C\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{L}\textcolor{black}{M}\textcolor{red}{N}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{M\ }\textcolor{green}{V}\textcolor{red}{P}\textcolor{red}{P}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{N}\textcolor{red}{N}\textcolor{green}{T}\textcolor{red}{S}\textcolor{green}{F}\textcolor{green}{D}\textcolor{red}{G}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{W}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{W}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{R\ }\\
\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{T\ }\textcolor{red}{G}\textcolor{green}{V}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{I}\textcolor{red}{F}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{I\ }\textcolor{red}{A}\textcolor{green}{G}\textcolor{black}{Y}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{S}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{N}\textcolor{green}{D\ }\textcolor{green}{R}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{V\ }\textcolor{green}{F}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{L}\textcolor{black}{Y\ }\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{A}\textcolor{red}{R}\textcolor{red}{F}\textcolor{red}{W}\textcolor{green}{F}\textcolor{green}{L}\textcolor{black}{C\ }\textcolor{green}{G}\textcolor{green}{A}\textcolor{red}{I}\textcolor{black}{M}\textcolor{red}{T}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{M\ }\textcolor{green}{V}\textcolor{red}{V}\textcolor{red}{S}\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{P\ }\textcolor{green}{N}\textcolor{red}{V}\textcolor{green}{T}\textcolor{red}{R}\textcolor{green}{F}\textcolor{green}{D}\textcolor{red}{R}\textcolor{green}{F}\textcolor{green}{R}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{I}\textcolor{black}{C}\textcolor{green}{I}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{S}\textcolor{green}{V\ }\textcolor{green}{W}\textcolor{green}{S}\textcolor{green}{G}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{W}\textcolor{green}{F}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{R\ }\\
\\
\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{G}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{G}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{T}\textcolor{green}{G}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/U9ZSQ2.tex <==


ID = U9ZSQ2



Description = Glycoside/pentoside/hexuronide transporter n=3 Tax=Escherichia coli TaxID=562 RepID=U9ZSQ2\_ECOLX

Length = 479 (aa)

Predicted matches = 291 / 404 (72.03\%)

TM-score = 0.7367

Superposition in the TM-score: Length(d<5.0)= 307

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/U9ZSQ2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{S}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{black}{M}\textcolor{red}{I}\textcolor{black}{Y}\textcolor{red}{I}\textcolor{green}{S}\textcolor{red}{I\ }\textcolor{red}{L}\textcolor{red}{A}\textcolor{black}{Y}\textcolor{red}{A}\textcolor{red}{D}\textcolor{black}{K}\textcolor{red}{T}\textcolor{black}{K}\textcolor{red}{N}\textcolor{black}{M\ }\textcolor{black}{K}\textcolor{red}{P}\textcolor{green}{E}\textcolor{red}{P}\textcolor{green}{L}\textcolor{green}{S}\textcolor{red}{I}\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{K\ }\textcolor{green}{I}\textcolor{red}{F}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{M}\textcolor{red}{V}\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{A\ }\textcolor{red}{W}\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{D}\textcolor{red}{I}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{black}{Y\ }\textcolor{black}{M}\textcolor{black}{M}\textcolor{red}{L}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{red}{N}\textcolor{green}{D}\textcolor{green}{I}\textcolor{red}{E}\textcolor{green}{G\ }\textcolor{green}{I}\textcolor{green}{P}\textcolor{red}{P}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{T}\textcolor{black}{M}\textcolor{red}{L\ }\textcolor{red}{E}\textcolor{green}{V}\textcolor{green}{A}\textcolor{red}{I}\textcolor{red}{Q}\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{A}\textcolor{red}{F}\textcolor{green}{S\ }\textcolor{green}{D}\textcolor{green}{P}\textcolor{black}{C}\textcolor{black}{M}\textcolor{green}{G}\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{W}\textcolor{red}{V}\textcolor{green}{R\ }\textcolor{red}{V}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{W}\textcolor{red}{S}\textcolor{black}{K}\textcolor{red}{T}\textcolor{green}{R}\textcolor{red}{L\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{red}{A}\textcolor{red}{L\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{V}\textcolor{black}{Y}\textcolor{black}{K}\textcolor{black}{M}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{red}{R}\textcolor{green}{S}\textcolor{red}{Q\ }\textcolor{red}{H}\textcolor{red}{P}\textcolor{black}{Y}\textcolor{red}{S}\textcolor{red}{I}\textcolor{black}{K}\textcolor{red}{E}\textcolor{black}{K}\textcolor{red}{Q}\textcolor{black}{M\ }\textcolor{black}{K}\textcolor{red}{S}\textcolor{green}{E}\textcolor{red}{V}\textcolor{green}{L}\textcolor{green}{S}\textcolor{red}{V}\textcolor{black}{K}\textcolor{green}{E}\textcolor{black}{K\ }\textcolor{green}{I}\textcolor{red}{G}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{black}{M}\textcolor{red}{G}\textcolor{red}{D}\textcolor{green}{A}\textcolor{green}{A}\textcolor{red}{S\ }\textcolor{red}{H}\textcolor{red}{I}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{D}\textcolor{red}{N}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{L}\textcolor{black}{Y\ }\textcolor{black}{M}\textcolor{black}{M}\textcolor{red}{F}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{red}{T}\textcolor{green}{D}\textcolor{green}{I}\textcolor{red}{F}\textcolor{green}{G\ }\textcolor{green}{I}\textcolor{green}{P}\textcolor{red}{A}\textcolor{green}{G}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{T}\textcolor{black}{M}\textcolor{red}{F\ }\textcolor{red}{L}\textcolor{green}{V}\textcolor{green}{A}\textcolor{red}{R}\textcolor{red}{A}\textcolor{green}{L}\textcolor{red}{D}\textcolor{green}{A}\textcolor{red}{I}\textcolor{green}{S\ }\textcolor{green}{D}\textcolor{green}{P}\textcolor{black}{C}\textcolor{black}{M}\textcolor{green}{G}\textcolor{red}{L}\textcolor{green}{L}\textcolor{red}{A}\textcolor{red}{D}\textcolor{green}{R\ }\textcolor{red}{T}\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{R}\textcolor{green}{W}\textcolor{red}{G}\textcolor{black}{K}\textcolor{red}{F}\textcolor{green}{R}\textcolor{red}{P\ }\textcolor{red}{W}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{P}\textcolor{red}{F}\textcolor{red}{G\ }\\
\\
\textcolor{green}{I}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{F}\textcolor{green}{P\ }\textcolor{green}{D}\textcolor{red}{V}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{I}\textcolor{black}{Y\ }\textcolor{red}{F}\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{V\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{red}{I}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{black}{C\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{G}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{P\ }\textcolor{red}{S}\textcolor{red}{E}\textcolor{red}{F}\textcolor{red}{S}\textcolor{green}{S}\textcolor{red}{F}\textcolor{red}{L}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{R\ }\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{A}\textcolor{red}{R}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{red}{F}\textcolor{green}{T}\textcolor{red}{D}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{L\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{red}{S}\textcolor{green}{Q}\textcolor{red}{T}\textcolor{red}{V}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{V\ }\textcolor{red}{S}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{H}\textcolor{green}{F}\textcolor{black}{C}\textcolor{green}{F\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{I}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{red}{T}\textcolor{green}{P\ }\textcolor{green}{D}\textcolor{red}{L}\textcolor{green}{S}\textcolor{black}{M}\textcolor{green}{N}\textcolor{green}{G}\textcolor{black}{K}\textcolor{black}{M}\textcolor{green}{I}\textcolor{black}{Y\ }\textcolor{red}{A}\textcolor{red}{A}\textcolor{green}{I}\textcolor{green}{T}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{L\ }\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{V}\textcolor{green}{N}\textcolor{green}{I}\textcolor{green}{P}\textcolor{black}{Y}\textcolor{black}{C\ }\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{G}\textcolor{green}{V}\textcolor{red}{I}\textcolor{green}{T}\textcolor{green}{N}\textcolor{green}{D}\textcolor{green}{P\ }\textcolor{red}{T}\textcolor{red}{Q}\textcolor{red}{R}\textcolor{red}{I}\textcolor{green}{S}\textcolor{red}{L}\textcolor{red}{Q}\textcolor{green}{S}\textcolor{green}{W}\textcolor{green}{R\ }\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{T}\textcolor{green}{A}\textcolor{red}{G}\textcolor{green}{G}\textcolor{black}{M}\textcolor{green}{L\ }\textcolor{red}{S}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{L}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{N\ }\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{D}\textcolor{green}{N}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{G\ }\textcolor{red}{F}\textcolor{green}{Q}\textcolor{red}{G}\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{V\ }\textcolor{red}{V}\textcolor{green}{A}\textcolor{green}{F}\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{F}\textcolor{black}{C}\textcolor{green}{F\ }\\
\\
\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{P\ }\textcolor{red}{L}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T}\textcolor{red}{T}\textcolor{black}{M}\textcolor{red}{G}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{red}{I}\textcolor{green}{D}\textcolor{red}{F}\textcolor{green}{W}\textcolor{red}{W}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{E}\textcolor{red}{L}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{red}{L}\textcolor{red}{R}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{A}\textcolor{green}{I}\textcolor{green}{F}\textcolor{red}{P}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M\ }\textcolor{black}{M}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{red}{N}\textcolor{green}{W}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{G}\textcolor{red}{T\ }\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{V}\textcolor{red}{S}\textcolor{green}{V}\textcolor{red}{L}\textcolor{green}{F}\textcolor{red}{T}\textcolor{red}{V}\textcolor{green}{T\ }\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{red}{V}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{E}\textcolor{green}{W}\textcolor{black}{K}\textcolor{black}{C\ }\textcolor{black}{K}\textcolor{green}{V}\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{F}\textcolor{red}{S}\textcolor{green}{W}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{A\ }\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{F\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{T}\textcolor{black}{K}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{green}{E}\textcolor{green}{A}\textcolor{green}{P\ }\textcolor{red}{P}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{T}\textcolor{red}{S}\textcolor{black}{M}\textcolor{red}{R}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{L\ }\textcolor{red}{R}\textcolor{green}{D}\textcolor{red}{I}\textcolor{green}{W}\textcolor{red}{Q}\textcolor{green}{N}\textcolor{green}{D}\textcolor{red}{Q}\textcolor{red}{W}\textcolor{green}{R\ }\textcolor{green}{I}\textcolor{red}{V}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{F}\textcolor{red}{N}\textcolor{green}{I\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{R}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{black}{M\ }\textcolor{black}{M}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{W}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{G}\textcolor{red}{S\ }\textcolor{green}{P}\textcolor{green}{E}\textcolor{green}{V}\textcolor{red}{F}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{F}\textcolor{red}{L}\textcolor{red}{T}\textcolor{green}{T\ }\textcolor{black}{Y}\textcolor{black}{C}\textcolor{green}{V}\textcolor{green}{G}\textcolor{green}{N}\textcolor{green}{L}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{S}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{red}{A}\textcolor{black}{K}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{T}\textcolor{red}{D}\textcolor{green}{W}\textcolor{black}{K}\textcolor{black}{C\ }\textcolor{black}{K}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{I}\textcolor{green}{F}\textcolor{red}{W}\textcolor{green}{W}\textcolor{green}{T}\textcolor{red}{N}\textcolor{green}{A\ }\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{black}{M}\textcolor{green}{F\ }\\
\\
\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{M}\textcolor{red}{D}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I}\textcolor{red}{N}\textcolor{black}{M\ }\textcolor{red}{I}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{V\ }\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{T}\textcolor{red}{I}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{W}\textcolor{black}{C}\textcolor{red}{I}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{red}{V}\textcolor{red}{P}\textcolor{green}{G}\textcolor{red}{N}\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{T}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{G}\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{W}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{D}\textcolor{black}{Y}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{I}\textcolor{green}{S}\textcolor{red}{A}\textcolor{red}{F}\textcolor{green}{I}\textcolor{red}{T}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{red}{W}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{A\ }\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{P}\textcolor{black}{M}\textcolor{red}{Q}\textcolor{green}{A}\textcolor{green}{S}\textcolor{green}{I}\textcolor{red}{T}\textcolor{black}{M\ }\textcolor{red}{F}\textcolor{green}{V}\textcolor{green}{F}\textcolor{green}{I}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{I}\textcolor{green}{G}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{V}\textcolor{red}{T}\textcolor{green}{P}\textcolor{green}{I}\textcolor{green}{Q}\textcolor{green}{W}\textcolor{green}{V\ }\textcolor{black}{M}\textcolor{black}{M}\textcolor{green}{S}\textcolor{green}{D}\textcolor{green}{T}\textcolor{red}{V}\textcolor{green}{D}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{green}{E\ }\textcolor{green}{W}\textcolor{black}{C}\textcolor{red}{N}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{G}\textcolor{green}{I\ }\textcolor{green}{S}\textcolor{red}{F}\textcolor{red}{A}\textcolor{green}{G}\textcolor{red}{T}\textcolor{red}{L}\textcolor{green}{F}\textcolor{green}{V}\textcolor{green}{L}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{red}{G}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{F}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{I\ }\textcolor{green}{G}\textcolor{green}{W}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{A}\textcolor{black}{Y}\textcolor{green}{G}\textcolor{red}{G}\textcolor{black}{Y}\textcolor{green}{D\ }\textcolor{green}{A}\textcolor{green}{A}\textcolor{green}{E}\textcolor{black}{K}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{N}\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{T\ }\textcolor{green}{I}\textcolor{green}{S}\textcolor{red}{I}\textcolor{red}{I}\textcolor{green}{I}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{I\ }\textcolor{green}{V}\textcolor{green}{P}\textcolor{green}{A}\textcolor{green}{I}\textcolor{black}{C}\textcolor{black}{Y}\textcolor{red}{L}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{A\ }\\
\\
\textcolor{red}{R}\textcolor{green}{I}\textcolor{red}{S}\textcolor{black}{K}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{N}\textcolor{red}{A}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{E}\textcolor{red}{T\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{red}{E}\textcolor{green}{F}\textcolor{green}{T}\textcolor{red}{F}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{S}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ \ }\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\\
\textcolor{red}{I}\textcolor{green}{I}\textcolor{red}{A}\textcolor{black}{K}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{black}{Y}\textcolor{green}{S}\textcolor{green}{L}\textcolor{green}{T\ }\textcolor{green}{T}\textcolor{green}{H}\textcolor{green}{N}\textcolor{red}{L}\textcolor{black}{K}\textcolor{green}{T}\textcolor{green}{V}\textcolor{black}{M}\textcolor{green}{E}\textcolor{red}{Q\ }\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{black}{K}\textcolor{green}{R}\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{Q}\textcolor{green}{Q\ }\textcolor{red}{Q}\textcolor{green}{F}\textcolor{green}{T}\textcolor{red}{S}\textcolor{green}{Q}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{Q}\textcolor{red}{N}\\
\\
\end{spacing}
}

\hrule


==> Alphafold/V0SJC2.tex <==


ID = V0SJC2



Description = Transcriptional regulator, TetR family n=3 Tax=Escherichia coli TaxID=562 RepID=V0SJC2\_ECOLX

Length = 199 (aa)

Predicted matches = 126 / 174 (72.41\%)

TM-score = 0.9047

Superposition in the TM-score: Length(d<5.0)= 189

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{Alphafold/V0SJC2.png}
\caption{Left: AlphaFold structures of predicted sequence (blue) and of UniProtKB (green). Center: AlphaFold structure of predicted sequence. Right: AlphaFold structure of UniProtKB sequence.}
\end{figure}

Alignment between predicted sequences and UniProtLB sequence:
 {
\begin{spacing}{0.5}
\ttfamily
\fontsize{7}{11}\selectfont
\texttt{}\\\textcolor{black}{M}\textcolor{red}{S}\textcolor{black}{K}\textcolor{red}{N}\textcolor{red}{G}\textcolor{red}{P}\textcolor{red}{W}\textcolor{red}{I}\textcolor{red}{R}\textcolor{red}{L\ }\textcolor{red}{T}\textcolor{red}{R}\textcolor{red}{E}\textcolor{red}{G}\textcolor{green}{L}\textcolor{red}{T}\textcolor{red}{I}\textcolor{red}{E}\textcolor{red}{A}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{N}\textcolor{red}{P}\textcolor{red}{E}\textcolor{red}{N}\textcolor{green}{I}\textcolor{green}{A}\textcolor{red}{H}\textcolor{red}{S\ }\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{V}\textcolor{red}{L}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{red}{A\ }\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{A}\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{A}\textcolor{green}{F}\textcolor{green}{W\ }\textcolor{green}{P}\textcolor{green}{D}\textcolor{black}{K}\textcolor{red}{R}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{red}{L}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{S}\textcolor{red}{E}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{red}{A}\textcolor{red}{V\ }\textcolor{green}{W}\textcolor{green}{R}\textcolor{red}{P}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{T\ }\textcolor{red}{S}\textcolor{green}{T}\textcolor{green}{A}\textcolor{red}{G}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{A\ }\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{N\ }\textcolor{red}{A}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{L}\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{A\ }\\
\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{\ }\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\\
\textcolor{black}{M}\textcolor{red}{G}\textcolor{black}{K}\textcolor{red}{T}\textcolor{red}{E}\textcolor{red}{E}\textcolor{red}{N}\textcolor{red}{S}\textcolor{red}{V}\textcolor{red}{Q\ }\textcolor{red}{R}\textcolor{red}{E}\textcolor{red}{D}\textcolor{red}{V}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{E}\textcolor{red}{A}\textcolor{red}{L}\textcolor{black}{K\ }\textcolor{green}{L}\textcolor{green}{L}\textcolor{red}{E}\textcolor{red}{L}\textcolor{red}{Q}\textcolor{red}{G}\textcolor{green}{I}\textcolor{green}{A}\textcolor{red}{N}\textcolor{red}{T\ }\textcolor{red}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{black}{M}\textcolor{green}{V}\textcolor{red}{A}\textcolor{green}{E}\textcolor{green}{R}\textcolor{green}{V}\textcolor{red}{D\ }\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{L}\textcolor{green}{D}\textcolor{red}{E}\textcolor{green}{L}\textcolor{green}{R}\textcolor{red}{R}\textcolor{green}{F}\textcolor{green}{W\ }\textcolor{green}{P}\textcolor{green}{D}\textcolor{black}{K}\textcolor{red}{E}\textcolor{green}{A}\textcolor{green}{I}\textcolor{green}{L}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{A\ }\textcolor{green}{L}\textcolor{red}{R}\textcolor{black}{Y}\textcolor{green}{L}\textcolor{green}{S}\textcolor{red}{Q}\textcolor{green}{Q}\textcolor{green}{I}\textcolor{red}{D}\textcolor{red}{A\ }\textcolor{green}{W}\textcolor{green}{R}\textcolor{red}{R}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{black}{M}\textcolor{green}{L}\textcolor{green}{D}\textcolor{green}{E}\textcolor{green}{T\ }\textcolor{red}{Q}\textcolor{green}{T}\textcolor{green}{A}\textcolor{red}{E}\textcolor{green}{Q}\textcolor{black}{K}\textcolor{green}{L}\textcolor{green}{L}\textcolor{green}{A}\textcolor{red}{R\ }\textcolor{black}{Y}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{L}\textcolor{green}{S}\textcolor{green}{E}\textcolor{black}{C}\textcolor{green}{V}\textcolor{black}{K}\textcolor{green}{N\ }\textcolor{red}{N}\textcolor{green}{R}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{L}\textcolor{red}{F}\textcolor{green}{I}\textcolor{green}{A\ }\\
\\
\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{T}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{H\ }\textcolor{red}{L}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{H}\textcolor{red}{I}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{D}\textcolor{red}{L}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{red}{R}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{L}\textcolor{red}{V}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{G}\textcolor{red}{H\ }\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{red}{E}\textcolor{green}{T}\textcolor{green}{A}\textcolor{red}{A\ }\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{A\ }\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{H}\\
\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:\ }\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\textcolor{black}{:}\\
\textcolor{green}{A}\textcolor{black}{C}\textcolor{green}{T}\textcolor{green}{F}\textcolor{black}{Y}\textcolor{green}{P}\textcolor{green}{D}\textcolor{green}{P}\textcolor{green}{G}\textcolor{green}{H\ }\textcolor{red}{P}\textcolor{green}{I}\textcolor{green}{H}\textcolor{green}{Q}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{Q}\textcolor{green}{Q}\textcolor{black}{K\ }\textcolor{green}{S}\textcolor{green}{A}\textcolor{green}{A}\textcolor{black}{Y}\textcolor{green}{D}\textcolor{green}{F}\textcolor{green}{T}\textcolor{green}{H}\textcolor{red}{E}\textcolor{green}{L\ }\textcolor{green}{L}\textcolor{green}{T}\textcolor{green}{T}\textcolor{green}{L}\textcolor{green}{E}\textcolor{green}{V}\textcolor{green}{D}\textcolor{red}{D}\textcolor{green}{P}\textcolor{green}{A\ }\textcolor{black}{M}\textcolor{green}{V}\textcolor{green}{A}\textcolor{black}{K}\textcolor{green}{Q}\textcolor{black}{M}\textcolor{green}{E}\textcolor{green}{L}\textcolor{green}{V}\textcolor{green}{L\ }\textcolor{red}{E}\textcolor{green}{G}\textcolor{black}{C}\textcolor{green}{L}\textcolor{red}{S}\textcolor{green}{R}\textcolor{black}{M}\textcolor{green}{L}\textcolor{red}{V}\textcolor{red}{N\ }\textcolor{green}{R}\textcolor{green}{S}\textcolor{green}{Q}\textcolor{green}{A}\textcolor{green}{D}\textcolor{green}{V}\textcolor{red}{D}\textcolor{green}{T}\textcolor{green}{A}\textcolor{red}{H\ }\textcolor{green}{R}\textcolor{green}{L}\textcolor{green}{A}\textcolor{green}{E}\textcolor{green}{D}\textcolor{green}{I}\textcolor{green}{L}\textcolor{green}{R}\textcolor{green}{F}\textcolor{green}{A\ }\textcolor{green}{R}\textcolor{black}{C}\textcolor{green}{R}\textcolor{green}{Q}\textcolor{green}{G}\textcolor{green}{G}\textcolor{green}{A}\textcolor{green}{L}\textcolor{red}{T}\\
\\
\end{spacing}
}

\hrule


==> texes/1-introduction-v1.tex <==
\section{Introduction}
The study of protein sequences, the fundamental building blocks of life, holds profound significance for humanity by offering insights into biological processes, disease mechanisms, and therapeutic developments. In this age of scientific renaissance, machine learning (ML), and particularly transformer models, have revolutionized the genomics and proteomics landscape. Originally designed for natural language processing, these models adeptly interpret the language of life encoded in protein sequences. They excel in predicting protein structures and functions, deciphering evolutionary relationships, and anticipating mutational impacts with remarkable performance. Their computational prowess offers boundless potential, bringing us closer to unlocking new possibilities in biotechnology and healthcare. However, despite decades of research, we have only scratched the surface in understanding the vast universe of proteins. Many proteins' structures, functions, and interactions remain unknown, representing a significant frontier in biology. This paper proposes an approach utilizing transformer models in conjunction with current experimental capabilities in protein sequencing. This method aims to practically accelerate the study of proteins through their sequences, enhancing our ability to gain deeper insights into complex biological processes and diseases via proteins.

In recent years, transformer models excel in learning representations from data, ranging from sequences to images and videos. For sequences data, models like BERT (Bidirectional Encoder Representations from Transformers)\cite{devlin2018bert} learn by masking a portion of words in a sentence and predicting them based on the attention to the surrounding context. During training, the model learns the dependencies between words and uses those relationships to understand their contexts and meanings, yielding accurate predictions of the masked words. This self--learning process allows BERT to grasp complex patterns and nuances from the data, making it especially helpful for understanding ``languages'' like genomics and proteomics. Existing application of transformers on protein sequences has been published by Rostlab in 2021\cite{9477085}. Their work demonstrates that their pretrained models can effectively learn the essences of protein sequences, achieving state--of--the--art performance in several protein general analysis tasks.


Transformer models' self--learning approach has inspired us to tackle the ongoing challenge of protein sequencing. While whole--genome sequencing platforms have achieved remarkable milestones in capacity and healthcare applications, protein sequencing remains constrained by issues of cost and precision. Developing efficient protein sequencing methods and building comprehensive proteomes would enable scientists to explore fundamental biological processes, from gene expression and protein translocation to post--translational modifications and frameshifting, as well as their roles in disease. Currently, the most established methods for sequencing proteins include mass spectrometry (MS)\cite{hunt1986protein}, liquid chromatography tandem mass spectrometry (LC MS/MS), and Edman degradation\cite{niall197336}\cite{alfaro2021emerging}. MS analyzes the mass--to--charge ratio of ionized particles to determine the protein's mass and sequence, but it often requires complex sample preparation and can struggle with large or highly modified proteins. LC MS/MS combines liquid chromatography to separate peptides with tandem mass spectrometry for detailed analysis, offering high sensitivity and throughput. However, this method is limited by its high cost, complex instrumentation, and inability to provide complete, high--throughput sequencing of full--length proteins. Lastly, Edman degradation sequentially removes and identifies amino acids from the protein's N--terminus, allowing step--by--step determination of the protein's sequence. While precise, it is slow and inefficient for long (no more than 70 residues) or blocked peptides. 

However, thanks for the development of click chemistry and bioorthogonal chemistry, recognized by the 2022 Nobel Prize in Chemistry, chemists are able to tag peptide fragments and label specific amino acids. Combining these novel techniques with traditional Edman degradation allows sequencing for peptides, providing per--residue index via cycle number tag and identification of specific amino acid types, limited to those that can be chemically labeled. Recent work by Zheng et al. has demonstrated the potential of this approach in sequencing short antibody peptides (10--30 residues in length), using labels for Phenylalanine (F), Tryptophan (W), Aspartic Acid (D), and Arginine (R)\cite{Zheng2024.05.31.596913}. Their study reported degradation efficiency well above 80\% and 100\% accuracy for canonical amino acids. In our opinions, if the C--terminus can be immobilized without peptide modification (on--going research), it is possible that we can cleave the protein into short peptides and sequence them efficiently, enabled full--length protein sequencing with targeted amino acids identified. The outcome of this combined approach yields a partially sequenced protein, similar to a masked protein sequence in transformer's learning task, but with targeted masking instead of random. This idea has inspired our work on applying BERT in fulfilling the missing information from the partially sequenced proteins, as well as their accuracy based on which known amino acids.

==> texes/2-background_study.tex <==
\section{Related Works}

\textbf{Overview of Protein Sequencing Technologies}
% This section seems like it will be a rehash of Introduction Section Paragraph 2? 
% More in depth talk about Edman Degredation & Mass Spectrometry? Not 100%


% Change title to 'Limitation of Current Sequencing Methods'? Remove existing in de novo as current de novo still has these constraints
\textbf{Limitation of Existing Sequencing}: Despite advancements in protein sequencing technologies, significant challenges persist. Bottom-up approaches, while widely used, are hindered by complex sample preparation and may miss critical modified peptides \cite{tubaon2017sample, mann2008precision}. Top-down and middle-down approaches offer advantages in proteoform characterization but are limited by incomplete sequence coverage \cite{fornelli2018top, toby2016progress}. Current characterization methods heavily rely on database searching, which proves inadequate for novel proteins or unexpected modifications \cite{anderson2017identification}. Existing de novo sequencing algorithms each have constraints: some require both top-down and bottom-up data \cite{liu2014novo}, others depend on specific fragmentation methods \cite{horn2000automated}, and some rely on pre-identified sequence tags \cite{vyatkina2015novo}. The exponential growth in possible amino acid sequences for gaps between fragments necessitates extremely high mass accuracy for unambiguous identification \cite{mann2008precision}. These limitations underscore the need for more robust and flexible methods for protein sequence analysis, particularly for novel or highly modified proteins.

\textbf{Advances in Computational Models}
% Recent advances in ... have significantly impacted protein sequencing.
% ML techniques .... to improve accuracy and efficiency
% Tools like AlphaFold ... brought unprecedented insights into protein folding and interactions {cite here}
% Pretrained language models such as ProtBert, ..., ProLlaMa has shown promise in predicting protein sequences from incomplete data, suggesting new approaches to overcome limitations of experimental techniques... {cite here, cite here}

\textbf{Integration of Machine Learning with Experimental Models}
% By simulating partial sequencing data, ML models can predict difficult to identify amino acids experimentally
% Bridges the gap between experimental limitations and computational predictions - provides better understanding of protein sequences
% (Example) ProtBert can predict masked residues in protein sequences, providing a scenario where experimental techniques could not identify some amino acids

\textbf{Gaps}


==> texes/6-discussion.tex <==
\section{Discussion}



